A Large Hadron Electron Collider at CERN: Report on the Physics and Design Concepts for Machine and Detector

The physics programme and the design are described of a new collider for particle and nuclear physics, the Large Hadron Electron Collider (LHeC), in which a newly built electron beam of 60 GeV, up to possibly 140 GeV, energy collides with the intense hadron beams of the LHC. Compared to HERA, the kinematic range covered is extended by a factor of twenty in the negative four-momentum squared, $Q^2$, and in the inverse Bjorken $x$, while with the design luminosity of $10^{33}$ cm$^{-2}$s$^{-1}$ the LHeC is projected to exceed the integrated HERA luminosity by two orders of magnitude. The physics programme is devoted to an exploration of the energy frontier, complementing the LHC and its discovery potential for physics beyond the Standard Model with high precision deep inelastic scattering measurements. These are designed to investigate a variety of fundamental questions in strong and electroweak interactions. The physics programme also includes electron-deuteron and electron-ion scattering in a $(Q^2, 1/x)$ range extended by four orders of magnitude as compared to previous lepton-nucleus DIS experiments for novel investigations of neutron's and nuclear structure, the initial conditions of Quark-Gluon Plasma formation and further quantum chromodynamic phenomena. The LHeC may be realised either as a ring-ring or as a linac-ring collider. Optics and beam dynamics studies are presented for both versions, along with technical design considerations on the interaction region, magnets and further components, together with a design study for a high acceptance detector. Civil engineering and installation studies are presented for the accelerator and the detector. The LHeC can be built within a decade and thus be operated while the LHC runs in its high-luminosity phase. It thus represents a major opportunity for progress in particle physics exploiting the investment made in the LHC.

==> detector/MagnetDesign.tex <==
%
%
\begin{table}[htp]
\begin{center}
\hspace*{-1.5cm}
\begin{tabular}{|c|c|c|c|c|c|c}
\hline 
     Option   &    Solenoid         & Dipole                     & Cryostat(s)     \\
              & $B= \hfill 3.5T$ &  $B= \hfill 0.3 T$         &                       \\
              &\hfill Length $= 570 cm$ & $L_{+z}= 600 cm$, \hfill  $L_{-z} = 370 cm$  &    Length = 1020 cm      \\
\hline\hline 
              &                          &                                         &                                   \\ 
 {\small\bf A}           &  $R_{min}= \hfill 90 cm$  & $R_{min}~~~~~~~~= \hfill 90 cm$ & EMC, Solenoid, Dipoles             \\ 
              &                  &  $R_{out_{Cryostat}}= \hfill 117.5 cm$   & $R_{in}= 48 cm$, \hfill $R_{out}=  117.5 cm$    \\
\hline\hline
              &                          &                                        &                                                \\ 
 {\small\bf B}         &$R^{1}_{min}= \hfill 230 cm$&               &   1$^{st}$-Solenoid                   \\ 
              &                          &   $\Delta{R_{Cryo-Sol_{out} }}   - \hfill $ not defined &     2$^{nd}$-Solenoid        \\
              &                         &                                         &                                                     \\ 
\hline
\end{tabular}
\end{center}
\caption{Magnet dimensions and characteristics of the two options {\small\bf A} and {\small\bf B} (no dipoles in case of Ring-Ring machine and in case B).}
\label{LHEC:MainDetector:MagnetDesign:table:1}
\end{table}
%
%
%
The main properties of the different magnet designs are summarised in Tabl.\,\ref{LHEC:MainDetector:MagnetDesign:table:1}. \\
%%Text beeing written by H.T.Kate, A.Dudarev - describing design properties etc.
%

==> machine/holzer.tex <==
\section{Interaction region layout}\label{layout}
\label{LHEC:machine:RR-IR-layout}
The design of the Interaction Region (IR) of the LHeC is particularly challenging as it 
has to consider boundary conditions from 
\begin{itemize}
\item{The lattice design and beam optics of the electron and proton beam}
\item{The geometry of the LHC experimental cavern and the tunnel} 
\item{The beam separation scheme which is determined by the bunch pattern of the LHC standard proton operation and related to this
 the optimization of the synchrotron light emission and collimation}
\item{The technical feasibility of the hardware.} 
\end{itemize}
%
Therefore the IR has to be optimized 
with respect to a well matched beam optics that adapts the optical parameters from the new electron-proton interaction point to the standard LHC proton beam 
optics in the arc and to the newly established beam optics of the electron ring. 
At the same time the two colliding beams as well as the non-colliding proton beam of LHC have to be separated efficiently and guided into their corresponding magnet lattices. 
As a general rule that has been established in the context of this study any modification in the standard LHC lattice and any impact 
on the LHC proton beam parameters had to be chosen moderately to avoid detrimental effects on the performance of the LHC proton-proton operation.
\par
The layout and parameters of the new e/p interaction point are defined by the particle physics requirements. At present the physics program 
that has been proposed for the LHeC ~\cite{Det_Acceptance} follows two themes - a high luminosity, high Q$^2$ program 
requiring a forward and backward detector acceptance of around 10$^{\circ}$ and a low x, low Q$^2$ program, which 
requires an increased detector acceptance  in forward and backward direction of at least 1$^{\circ}$ and could proceed with reduced luminosity.
 Accordingly two machine scenarios 
have been studied for the interaction region design. Firstly, a design that has been optimised for high luminosity 
with an acceptance of 10$^{\circ}$ and secondly, a high acceptance design that allows for a smaller opening angle of the detector. 
In both cases the goal for the machine luminosity is in the range 
of 10$^{33}\,\mathrm{cm}^{-1}\,\mathrm{s}^{-1}$ but the layouts differs in the magnet lattice, the achievable absolute luminosity and mainly the synchrotron 
radiation that is emitted during the beam separation process. 
Both options will be presented here in detail and the corresponding design luminosity, the technical requirements and the synchrotron radiation load will be compared. 
In both cases however, a well matched spot size of the electron and proton beam  had to be established at the collision point: Experience in SPS and 
HERA  \cite{Bieler:1999iz}\cite{Zimmermann:1992da} showed that 
matched beam cross sections have to be established between the two colliding beams to
 guarantee stable beam conditions.
Considering the different nature of the beams, namely the emittances of the electron beam in the two transverse planes, the interaction region design has to consider this boundary
 condition and the beam optics has to be established to achieve equal beam sizes  $ \sigma _x (p) = \sigma _x (e) $, $ \sigma _y (p) = \sigma _y (e)$  at the IP. 

The basic beam parameters however like energy, particle intensity and beam emittances  are identical for both designs, determined by the 
electron and proton ring lattices and the pre-accelerators. They are summarised in Table~\ref{tab:parameters}.

\begin{table}[h]
\begin{center}
\begin{tabular}{|l|c|c|c|}
\hline
Quantity                      &  unit   &     e    &   p        \\
\hline
Beam energy                   &  GeV    &    60    &  7000      \\
Total beam current            &   mA    &   100    &   860      \\
Number of bunches             &         &  2808    &  2808      \\
Particles/bunch $N_b$         &$10^{10}$&  2.0    &   17       \\
Horiz.\ emittance             &   nm    &   5.0    &  0.5       \\
Vert.\ emittance              &   nm    &   2.5    &  0.5       \\
%Energy loss per turn         &  GeV    & 0.707    &  $6\times10^{-6}$ \\
%Radiated power               &   MW    &    50    &  0.003     \\
\hline
Bunch distance                &   ns    & \multicolumn{2}{|c|}{25}     \\
\hline
\end{tabular}
\caption{Main parameters for e/p collisions.}
\label{tab:parameters}
\end{center}
\end{table}


Colliding two beams of different characteristics, the luminosity obtained is given by the equation
\begin{equation}
L=\sum_{i=1}^{n_b} ( I_e * I_p)\frac{1}{ e^2 f_0 2\pi \sqrt{ \sigma_{xp}^2 + \sigma_{xe}^2} \sqrt{ \sigma_{yp}^2 + \sigma_{ye}^2} },
\end{equation}
where $\sigma_{x,y}$  denotes the beam size of the electron and proton beam in the horizontal and vertical plane and $I_e$, $I_p$  the electron and proton 
single bunch currents. In all IR layouts, the proton beam size at the IP is matched to the electron beam size in order to optimise the delivered luminosity 
and minimise detrimental beam beam effects. 
\par

The main difference of the IR design for the electron proton collisions with respect to the existing LHC interaction regions is the fact that the two beams 
of LHeC cannot be focussed and / or guided at the same time: The different nature of the two beams, the fact that the electrons emit synchrotron radiation 
and mainly the large difference in the particle momentum make a simultaneous focusing of the two beams impossible. The strong gradients of the proton 
quadrupoles in the LHC triplet structure cannot be tolerated nor compensated for the electron lattice and a stable optical solution for the electrons is 
not achievable under the 
influence of the proton magnet fields. The electron beam therefore has to be separated from the proton beam after the collision point  before any strong `` 7 TeV like''  
magnet field is applied.  
\\ In order to obtain still a compact design and to optimize the achievable luminosity of the new e/p interaction region, the beam separation scheme has to be combined with the electron mini-beta focusing structure.
 
Figure \ref{Fig:IR_gross} shows a schematic layout of the interaction region. It refers to the 10 degree option and shows a compact triplet 
structure that is used for early focusing of the electron beam. The electron mini beta quadrupoles are embedded into the detector opening angle and in order to obtain the required separation effect they are shifted in the horizontal plane and  
act effectively as combined function magnets: Thus focusing and separation of the electron beam are combined in a very compact lattice structure, 
which is the prerequisite to achieve luminosity values in the range of $10^{33}$ cm $^{-2}$ s$^{-1}$. 
 
\begin{figure}
\centerline{\includegraphics[clip=,width=0.9\textwidth]{IR_gross.pdf}}
\caption{Schematic layout of the LHeC interaction region}
\label{Fig:IR_gross}
\end{figure}


\subsection{Beam separation scheme}

The separation scheme of the two beams has to be optimised with respect to an efficient (i.e. fast) beam separation 
and a synchrotron radiation power and critical energy of the emitted photons that can be tolerated by the absorber design. Two main issues 
have to be accomplished: a sufficient  horizontal distance between the beams has to be generated at the position of the first proton (half) quadrupole, located at 
a distance of s = 22m from the interaction point (the nominal value of the LHC proton lattice). In addition to that, harmful beam beam effects have to be avoided at the 
first   parasitic bunch encounters which will take place at s = 3.75m, as the nominal bunch distance in LHC corresponds to $\Delta t = 25ns$. 
These so-called parasitic bunch crossings have to be avoided as they would lead to intolerable beam-beam effects in the colliding beams. 
As a consequence the separation scheme has to deliver a sufficiently large horizontal distance between the two counter rotating bunches at these locations. 
\par
To achieve the first requirement a separation effect is created inside the mini beta quadrupoles of the electron beam:  
The large momentum difference of the two colliding beams provides a 
very elegant way to separate the lepton and the hadron beams:  Shifting the mini-beta quadrupoles of the electron beam and installing a 15.8m long, but 
weak separator dipole  magnet close to the IP provides the gentle separation that is needed to keep the synchrotron radiation level in the IR 
within reasonable limits. 
\\
The nearest proton quadrupole to the IP is designed as a half-quadrupole to ease the extraction of the outgoing electron beam. 
At this location (at s=22m) a minimum separation of $ \Delta x = $ 55mm  is needed to guide the electron beam along 
the mirror plate of a sc. proton half quadrupole (see Section $\ref{tripletmagnets}$).
A first layout of this magnet is sketched in figure \ref{Fig:half_quad}

\begin{figure}
\centerline{\includegraphics[clip=,width=0.55\textwidth]{half_quad.pdf}}
\caption{Super conducting half  quadrupole  in the proton lattice: The electron beam will pass on the right hand side of the mirror plate in 
a quasi field free region (see Section $\ref{tripletmagnets}$).}
\label{Fig:half_quad}
\end{figure} 


The horizontal offsets of the mini beta lenses are chosen individually in such a way that the resulting bending strength in the complete separation 
scheme (quadrupole triplet / doublet and separator dipole) is constant. In this way a moderate separation strength is created with a constant bending 
radius of $ \rho=6757m$ for the 10 degree option. 
In the case of the 1 degree option the quadrupole lenses of the electron lattice cannot be included
 inside the detector design as the opening angle of the detector does not provide enough space for the hardware of the electron ring lattice. Therefore a much 
larger distance between the IP and the location of the first electron lens had to be chosen ($\Delta $ s =6.2m instead of $\Delta $ s =1.2m).   
As a consequence - in order to achieve the same overall beam separation - stronger magnetic separation fields have to be applied resulting in a 
 bending radius of  $ \rho=4057m$ in this case. 
In both cases the position of the electron quadrupoles is following the design orbit of the electron beam to avoid local strong bending fields and keep the 
synchrotron radiation power to a minimum. This technique has already been succesfuly applied at the layout of the HERA electron-proton 
collider \cite{Rossbach:1985ve}. \\
 
Still the separation at the location of the first proton magnet is small and  a half quadrupole design for this super conducting magnet has  
been chosen at this point. The resulting beam parameters - including the expected  luminosity for this ring ring option - are summarised in Table 2.

 
\begin{table}
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Detector Option       &            &      \multicolumn{2}{|c|} { 1$^{\circ}$  }  &    \multicolumn{2}{|c|} {10$^{\circ}$ }    \\
Quantity              &     unit   &       electrons      &    protons           &     electrons      &            protons    \\
\hline
Number of bunches     &            &           \multicolumn{4}{|c|} {2808}                           \\
\hline
Particles/bunch $N_b$ & $10^{10}$  &          1.96        &         17            &           1.96    &                 17    \\
Horiz. beta-function  &   m        &           0.4        &        4.0            &           0.18    &                1.8    \\
Vert. beta-function   &   m        &           0.2        &        1.0            &            0.1    &                0.5    \\
Horiz.\ emittance     &  nm        &           5.0        &        0.5            &            5.0    &                 0.5   \\
Vert.\ emittance      &  nm        &           2.5        &        0.5            &            2.5    &                 0.5   \\
\hline
Distance to IP        &   m        &           6.2        &         22            &            1.2    &                  23   \\
\hline
Crossing angle        &  mrad      &           \multicolumn{2}{|c|} {1.0}         &      \multicolumn{2}{|c|} {1.0}           \\ 
Synch. Rad. in IR     &  kW        &           \multicolumn{2}{|c|} {51}          &      \multicolumn{2}{|c|} {33}            \\ 
\hline
absolute Luminosity   &cm$^{-2}$ s$^{-1}$&      \multicolumn{2}{|c|} {$8.54*10^{32}$ }&      \multicolumn{2}{|c|} {$1.8*10^{33}$} \\  
Loss-Factor S         &            &        \multicolumn{2}{|c|} {0.86}           &      \multicolumn{2}{|c|} {0.75}          \\  
effective Luminosity  &cm$^{-2}$ s$^{-1}$&      \multicolumn{2}{|c|} {$7.33*10^{32}$ }&      \multicolumn{2}{|c|} {$1.34*10^{33}$}\\    
\hline   
\end{tabular}
\caption{Parameters of the mini beta optics for the 1$^{\circ}$ and 10$^{\circ}$ options of the LHeC Interaction Region.}
\label{tab:IR_parameters}
\end{center}
\end{table}

It has to be pointed out in this context that the arrangement of the off centre quadrupoles as well as the strength of the separator dipole depend 
on the beam optics of the electron beam. The beam size at the parasitic crossings and at the proton quadrupole will determine the required 
horizontal distance between the electron and proton bunches.  The strength and position of these magnets however will determine the optical 
parameters, including the dispersion function that is created during the separation process itself.
Therefore a self-consistent layout concerning optics, beam separation and geometry of the synchrotron light absorbers has to be found. 

\par
It is obvious that these boundary conditions have to be fulfilled not only during luminosity operation of the e/p rings. During injection and the 
complete acceleration procedure of the electron ring the influence of the electron quadrupoles on the proton beam has to be compensated with respect to the proton beam 
orbit (as a result of the separation fields) as well as to the proton beam optics: The changing deflecting fields and gradients  of the electron magnets will 
require correction procedures in the proton lattice that will compensate this influence at any moment.  

\subsection{Crossing angle} 

A central aspect of the LHeC IR design is the beam-beam interaction of the colliding electron and proton bunches. The bunch structure of 
the electron beam will match the pattern of the LHC proton filling scheme for maximal luminosity, giving equal bunch spacings of 25 ns  to both beams. 
The IR design therefore is required to separate the bunches as quickly as possible to avoid additional bunch interactions at these positions and limit the 
beam-beam effect to the desired  
interactions at the IP. The design bunch distance in the LHC proton bunch chain corresponds 
to $ \Delta t$ =25 ns  or $\Delta$ s=7.5 m. The counter rotating bunches therefore meet after the crossing at the interaction point at additional, parasitic 
collision points in  
a distance s = 3.75 m from the IP.  To avoid detrimental effects from these parasitic crossings the above 
mentioned separation scheme has to be supported by a crossing angle that will deliver a sufficiently large horizontal distance between the bunches at the first 
parasitic bunch crossings. 
This technique is used in all LHC interaction points. In the case of the LHeC however, the crossing angle is determined by the emittance of the 
electron beam and the resulting beam size which is considerably larger than the usual proton beam size in the storage ring. In the case of the 
LHeC IR a crossing angle of $ \theta$ = 1mrad is considered as sufficient in the 1$^{\circ}$ as well as in the 10$^{\circ}$ option to avoid beam-beam effects from this parasitic crossings. 
Figure \ref{Fig:IR_zoom_bunche} shows the position of the first possible parasitic encounters and the effect of the crossing angle to deliver 
a sufficient separation at these places. 

The detailed impact of one beam on another is evaluated by a dedicated beam-beam interaction study which is included in this report, based on  a 
minimum separation of 5$\sigma_e + 5\sigma_p$ at every parasitic crossing node. Due to the larger electron emittance the separation is 
mainly dominated by the electron beam parameters, and as a general rule it can be stated that the rapid growth of
the $\beta$-function in the drift around the IP,
\begin{equation}
\beta(s)=\beta^* + \frac{s^2}{\beta^*},
\end{equation}
makes it harder  to separate the beams if small $\beta^*$ and a large drift space $s$ is required in the optical design.  

\begin{figure}
\centerline{\includegraphics[clip=,width=0.9\textwidth]{IR_zoom_3.pdf}}
\caption{LHeC interaction region including the location of the first parasitic bunch encounters where 
a sufficient beam separation is achieved by a crossing angle of 1 mrad. The location of the parasitic encounters is indicated by green ovals.}
\label{Fig:IR_zoom_bunche}
\end{figure}

In any design for the LHeC study, a crossing angle is used to establish an early beam separation, reduce the required strength in the separation magnets and minimise the 
synchrotron radiation power that is created inside the interaction region. 

As a draw back however  the luminosity 
is reduced  due to the fact that the bunches will not collide anymore head on.
This reduction is expressed in a geometric luminosity reduction factor ``S'', that depends on the crossing angle $ \theta$, the 
length of the electron and proton bunches $ \sigma_{ze} $ and $ \sigma_{zp} $ and the transverse beam size in the plane of 
the bunch crossing $ \sigma^*_x $:

\begin{equation}
S(\theta) = \left[1+\left(\frac{\sigma^2_{sp}+\sigma^2_{se}}{2\sigma^{*2}_x}\right)\tan^2\frac{\theta}{2}\right]^{-\frac{1}{2}}\ .
\label{eqn:S}
\end{equation}\\

Accordingly, the effective luminosity that can be expected for a given IR layout is obtained by 
\begin{equation}
L = S(\theta) * L_0
\end{equation}\\
  
For the two beam optics that have been chosen for this design study (the  1$^{\circ}$ and the  10$^{\circ}$ option) and a  crossing angle of $ \theta $ = 1mrad  the loss factor amounts to 
$S=74 \%$ and $S=85 \%$ respectively.

\subsection{Beam optics and luminosity}

A special boundary condition had to be observed in the design of the proton beam optics of the LHeC: For the layout of the four 
present proton-proton interaction regions in the LHC machine an anti-symmetric option had been chosen: A solution that is 
appropriate for a round beam optics ( $ {\sigma_x}^* = {\sigma_y}^* $ ). An optimised design for collisions with the flat e$^{\pm} $  
beams however requires unequal $ \beta $ -functions for the hadron beam at the IP and the existing LHC optics can no longer be maintained. 
Therefore the optical layout of the existing triplet structure in the LHC had to be modified to match the required beta 
functions ( $ \beta_x$ = 1.8m, $\beta_y$ = 0.5m) at the IP  to the regular optics of the FODO structure in the arc (Figure \ref{Fig:lhec_p_optik}).

\begin{figure}
\centerline{\includegraphics[clip=,width=0.65\textwidth]{lhec_p_optik.pdf}}
\caption{Proton optics for the LHeC interaction region. The gradients of the antisymmetric triplet lattice in the standard LHC have been modified to adopt 
for the requirements of the LHeC flat beam parameters.}
\label{Fig:lhec_p_optik}
\end{figure}


In the case of the electron beam optics, two different layouts of the interaction region are considered: One optical concept for highest achievable 
luminosity and a solution for maximum detector acceptance.   
In the first case an opening angle of  10$^{\circ}$ is available inside the detector geometry and  allows to install an embedded 
magnet structure where the first electron quadrupole lenses can be placed as close as 
$s $= 1.2m  from the IP. This early focusing scheme leads to moderate values of the $ \beta $ function inside the mini beta quadrupoles 
and therefore allows for a smaller spot size at the IP and larger luminosity values can be achieved. Still however the quadrupoles require a 
compact design: While the gradients required by the optical solution are small (for a super conducting magnet design) the outer radius of the 
first electron quadrupole has been limited to $ r_{max}$ = 210mm.

\begin{figure}
\centerline{\includegraphics[clip=,width=0.65\textwidth]{lhec_e_optik.pdf}}
\caption{Electron optics for the LHeC interaction region. The plot corresponds to the 10 degree option where a triplet structure combined with a 
separation dipole has been chosen to separate the two beams.}
\label{Fig:lhec_e_optik}
\end{figure}

In the case of the 1$^{\circ}$ option the detector design is optimised for largest detector acceptance. Accordingly the opening angle of the 
detector hardware is too small to deliver space for accelerator magnets. The mini beta quadrupoles therefore have to be located outside the detector, 
and  a distance $s$ = 6m from the IP had to be chosen in this case. Even if the magnet dimensions are not limited by the detector design in this case, the achievable 
luminosity is about a factor of two smaller than in the 10$^{\circ}$ case.  



The two beam optics that are based on these considerations are discused in detail in the next chapter of this report. 
In the case of the 10$^{\circ}$ option a triplet structure has been chosen to allow for moderate values of the beta functions inside 
the mini beta quadrupoles. As a special feature of the optics that is shown in Figure \ref{Fig:lhec_e_optik} the focusing effect of the first 
quadrupole magnet is moderate: Its gradient has been limited as it has to deliver mainly the first beam separation. 
 Table~\ref{tab:IR_parameters} includes as well the overall synchrotron radiation power that is produced inside the IR. Due to the larger bending 
radius (i.e. smaller bending forces) in the case of the  10$^{\circ}$ option the produced synchrotron radiation power is limited to about 30 kW, 
while the alternative - high acceptance - option has to handle 50kW of synchrotron light.\\
The details of the synchrotron light characteristics   are covered in the next chapters of this report for both cases, including the critical energies 
and the  design of the required absorbers. 

For the 1$^{\circ}$ option the mini beta focusing is based on a quadrupole doublet as the space limitations in the transverse plane 
are much more relaxed compared to the alternative option and the main issue here was to find  a compact design in the longitudinal coordinate: 
Due to the larger distcance of the focusing and separating magnets from the IP the magnet structure has to be more compact and the 
separating field stronger to obtain the required horizontal beam distance at the location s=22m of the first proton quadrupole. 
The corresponding beam optics for both options are explained in full detail below.  


==> machine/luke_thompson.tex <==

%
% found that these section headlines seem not needed (MKlein 29.7.)
%\section{Design Requirements of the Electron Beam Optics}
%\label{IR.Design}
%
%\subsection{Optics Matching and IR Geometry}
%\label{IR.Design.LM}

Once the beams are separated into independent beam pipes, the electron beam must be transported into the ring lattice. Quadrupoles are used in the electron machine LSS to transport the beam from the IP to the dispersion suppressor and match twiss parameters at either end. This matching must be smooth and not require unfeasible apertures. In addition the first electron quadrupoles will be located inside the detector hardware and therefore a compact design is required within the limited space available.  \\

The complete design of the long straight section  "LSS", that includes the mini beta insertion, the matching section  and the dispersion suppressor must be designed around a number of further constraints. As well as beam separation, the electron beam must be steered from the electron ring into the IR and back out again. The colliding proton beam must be largely undisturbed by the electron beam. The non-colliding proton beam must be guided through the IR without interacting with either of the other beams.

\subsection{High luminosity IR layout}
\label{IR.HL}

\subsubsection{Parameters}
\label{IR.HL.P}
Table \ref{tab:IR.HL.P.Params} details the interaction point parameters and other parameters for this design. To optimise for luminosity, a small $l$* is desired. An acceptance angle of 10\textdegree~is therefore chosen, which gives an $l$* of 1.2m for final focusing quadrupoles of reasonable size.


\begin{table}[!h]
\begin{centering}
\begin{tabular}{|l|l|}
	\hline
	$L(0)$&1.8$\times 10^{33}$\\ \hline
	$\theta$&1$\times 10^{-3}$\\ \hline
	$S(\theta)$&0.746\\ \hline
	$L(\theta)$&1.34$\times 10^{33}$\\ \hline
	$\beta_x*$&0.18 m\\ \hline
	$\beta_y*$&0.1 m\\ \hline
	$\sigma_x*$&3.00$\times 10^{-5}$ m\\ \hline
	$\sigma_y*$&1.58$\times 10^{-5}$ m\\ \hline
	SR Power&33 kW\\ \hline
	$E_c$&126 keV\\ \hline
\end{tabular}
\caption{Parameters for the High Luminosity IR.}
\label{tab:IR.HL.P.Params}
\end{centering}
\end{table}


\noindent SR calculations are detailed in Section\,\ref{NATHAN}. The total power emitted in the IR is similar to that in the HERA-2 IR [reference] and as such appears to be reasonable, given enough space for absorbers.

\subsubsection{Layout}
\label{IR.HL.L}
Due to the relatively round beam spot aspect ratio of 1.8:1, a final quadrupole triplet layout has been chosen for this design. The relatively weak horizontal focusing quadrupole used as first magnet lens is mainly needed for beam separation, followed by two strong, nearly doublet like quadrupoles.   The focusing strength Figure \ref{fig:IR.HL.L.Layout} and table \ref{tab:IR.HL.L.Layout} detail the layout.\\

\begin{figure*}[!h]
\begin{center}
\includegraphics[scale=0.6]{10_Layout.pdf}
\caption{Layout of machine elements in the High Luminosity IR. Note that the left side of the IR is symmetric.}
\label{fig:IR.HL.L.Layout}
\end{center}
\end{figure*}

\begin{table}[!h]
\begin{centering}
\begin{tabular}{|l|l|l|l|l|l|l|}
	\hline
	Element&S$_{entry}$ [m]&L [m]&Gradient [T/m]&Dipole Field [T]&Offset [m]\\ \hline\hline
	BS.L&-21.5&15.8&-&-0.0296&-\\ \hline
	Q3E.L&-5.4&1.0&89.09229&-0.0296&-3.32240$\times 10^{-4}$\\ \hline
	Q2E.L&-4&1.5&-102.2013&-0.0296&2.89624$\times 10^{-4}$\\ \hline
	Q1E.L&-2.2&1.0&54.34071&-0.0296&-5.44711$\times 10^{-4}$\\ \hline
	IP&0.0&-&-&-&-\\ \hline
	Q1E.R&1.2&1.0&54.34071&0.0296&5.44711$\times 10^{-4}$\\ \hline
	Q2E.R&2.5&1.5&-102.2013&0.0296&-2.89624$\times 10^{-4}$\\ \hline
	Q3E.R&4.4&1.0&89.09229&0.0296&3.32240$\times 10^{-4}$\\ \hline
	BS.R&5.7&15.8&-&-0.0296&-\\ \hline
\end{tabular}
\caption{Machine elements for the High Luminosity IR. S$_{entry}$ gives the leftmost point of the idealised magnetic field of an element. Note that S is relative to the IP.}
\label{tab:IR.HL.L.Layout} 
\end{centering}
\end{table}


\noindent The $l$* of 1.2 m allows both strong focusing of the beam, and constant bending of the beam from 1.2 m to 21.5 m. This is achieved with offset quadrupoles and a separation dipole.\\
\\
Figure \ref{fig:IR.HL.L.Twiss} shows the $\beta$ functions of the beam in both planes from the IP to the face of the final proton quadrupole at s~=~23~m.

\begin{figure*}[!h]
\begin{center}
\includegraphics[scale=0.5]{10_IP_smooth.pdf}
\caption{$\beta$ functions in both planes for the High Luminosity IR layout, from the IP to the face of the final proton quadrupole at s~=~23~m. Note that s is relative to the ring, which begins at the left side of the left dispersion suppressor of IP2.}
\label{fig:IR.HL.L.Twiss}
\end{center}
\end{figure*}

\subsubsection{Separation scheme}
\label{IR.HL.S}
As described above a quadrupole triplet configuration is used for the first focusing of the electron beam. This has the effect of generating a larger peak in $\beta_x$, between parasitic crossings but leads to smaller horizontal beam sizes at these locations and therefore reduces the necessary beam separation. The first F quadrupole reduces $\beta_x$ at s~=~3.75~m compared to an initial D quadrupole. The third F quadrupole then brings $\beta_x$ down from the peak sufficiently to avoid large beam-beam interactions at the second parasitic crossing, s~=~7.5~m.\\
\\
Separation is provided by the bending effect of the offset quadrupoles, and also the IP crossing angle of 1~mrad. These elements ensure that the separation between the beams, normalised to beam size, increases at each parasitic crossing. Note that 1~mrad is not a minimum crossing angle required by beam-beam interaction separation criteria; it is however a chosen balance between luminosity loss and minimising bend strength. In theory, this layout could support an IP with no crossing angle; however the bend strength required to achieve this would generate an undesirable level of SR power.

\subsubsection{Optics matching and IR geometry}
\label{IR.HL.LM}
The IR is matched into the ring arc lattice by means of matching quads in the LSS. The quads are roughly evenly placed, with sufficient space left after the IR section to accommodate the proton optics and the remaining electron ring geometry, which has yet to be designed fully. The solution is nearly symmetric about the IP; however due to the geometry of the LHC lattice, the electron ring itself is not exactly symmetric. As such the solution differs slightly on either side of the LSS. Table \ref{tab:IR.HL.LM.Layout} details the layout of machine elements in the LSS. Five matching quadrupoles are used on either side of the IP. A sixth quadrupole is used on the left side, next to the dispersion suppressor. Due to the asymmetric design of the dispersion suppressors, a quadrupole (MQDSF.L2) is included at the same distance from the IP on the right side as part of the dispersion suppressor. MQDSF.L2 is required to match the optics, but is more constrained than the other matching quadrupoles. Figure \ref{fig:IR.HL.LM.TwissLR} shows the $\beta$ functions of the matching from the IP to the dispersion suppressor, on both sides of the IP (Figure \ref{fig:IR.HL.LM.TwissR})\\

\begin{table}
\centering
\begin{tabular}{|l|l|l|l|}
	\hline
	Element&S$_{entry}$ [m]&L [m]&Gradient [T/m]\\ \hline
	MQDSF.L2&-268.8944&1.0&8.451030\\ \hline
	MQDM5.L2&-240.5&1.0&-7.306991\\ \hline
	MQFM4.L2&-199.5&1.0&6.529028\\ \hline
	MQDM3.L2&-162.5&1.0&-6.561684\\ \hline
	MQFM2.L2&-120.5&1.0&6.140239\\ \hline
	MQDM1.L2&-82.5&1.0&-5.127192\\ \hline
	MQDM1.R2&81.5&1.0&-5.286055\\ \hline
	MQFM2.R2&119.5&1.0&6.171258\\ \hline
	MQDM3.R2&161.5&1.0&-6.641329\\ \hline
	MQFM4.R2&198.5&1.0&7.058192\\ \hline
	MQDM5.R2&239.5&1.0&-7.26769\\ \hline	
\end{tabular}
\caption{Machine elements for the High Luminosity LSS layout. S$_{entry}$ gives the leftmost point of the idealised magnetic field of an element. Note that S is relative to the IP.}
\label{tab:IR.HL.LM.Layout}
\end{table}

\begin{figure*}[!h]
\begin{center}
\includegraphics[scale=0.5]{10_LSS_smooth.pdf}
\caption{$\beta$ functions in both planes for the High Luminosity IR layout, from the end of the left dispersion suppressor to the start of the right dispersion suppressor. Note that s is relative to the ring, which begins at the left side of the left dispersion suppressor of IP2.}
\label{fig:IR.HL.LM.TwissLR}
\end{center}
\end{figure*}

\begin{figure*}[!h]
\begin{center}
\includegraphics[scale=0.5]{10_LSSR_smooth.pdf}
\caption{$\beta$ functions in both planes for the High Luminosity IR layout, from the IP to the start of the right dispersion suppressor. Note that s is relative to the ring, which begins at the left side of the left dispersion suppressor of IP2.}
\label{fig:IR.HL.LM.TwissR}
\end{center}
\end{figure*}

\noindent A smooth matching is obtained, where the maximum beta functions are well controlled and continuously reduced to the values of the  arc structure. The beam envelopes in the LSS are of reasonable size and do not require excessive aperture.\\
\\
Note that this solution is not yet matched for dispersion as the rest of the ring geometry in the LSS and IR areas is yet to be designed. 

\begin{figure*}[!h]
\begin{center}
\includegraphics[scale=0.6]{LSS_Geom.pdf}
\caption{Graphical representation of misaligned LSS/IR geometry. With beam steering in the IR and no compensation in the LSS, the electron beam no longer lines up with the ring lattice reference orbit. Diagram is not to scale and does not represent the correct optical layout of the IR nor the LSS.}
\label{fig:IR.HL.LM.Orbit}
\end{center}
\end{figure*}

\noindent Plans for the remaining IR geometry include a second horizontal dipole, and quadrupoles, on either side to turn each separation dipole into a dispersion-free S-shaped bend. This will be used to extract the beam into the electron machine. 

\subsection{High acceptance IR layout}
\label{IR.HA}

\subsubsection{Parameters}
\label{IR.HA.P}
Table \ref{tab:IR.HA.P.Params} details the design parameters for this option. The chosen detector opening angle for this layout is 1\textdegree. All elements, especially the mini beta quadrupoles of the electron ring, therefore have to be placed  outside the limits of the detector, at $z = \pm6.2$m, where $z$ the is longitudinal axis of the detector.  As such, the actual acceptance of the layout is limited by the beam pipe rather than the size of machine elements. This also gives further flexibility in the strengths and designs of the final focusing quadrupoles, although this flexibility is not exploited in the design.\\

\begin{table}[!h]
\centering
\begin{tabular}{|l|l|}
	\hline
	$L(0)$&8.54$\times 10^{32}$\\ \hline
	$\theta$&1$\times 10^{-3}$\\ \hline
	$S(\theta)$&0.858\\ \hline
	$L(\theta)$&7.33$\times 10^{32}$\\ \hline
	$\beta_x*$&0.4 m\\ \hline
	$\beta_y*$&0.2 m\\ \hline
	$\sigma_x*$&4.47$\times 10^{-5}$ m\\ \hline
	$\sigma_y*$&2.24$\times 10^{-5}$ m\\ \hline
	SR Power&51 kW\\ \hline
	$E_c$&163 keV\\ \hline
\end{tabular}
\caption{Parameters for the High Acceptance IR.}
\label{tab:IR.HA.P.Params}
\end{table}

\noindent SR calculations are discussed in detail in Section\,\ref{NATHAN}. The total power emitted in the IR is similar to that in the HERA-2 IR [reference] and as such appears to be reasonable, given enough space for absorbers. However it is significantly higher than that in the high luminosity layout. As discussed in Section\,\ref{NATHAN}, an option exists to reduce the total SR power by including a dipole field in the detector, thus mitigating the limitation imposed on dipole length by the larger $l$*.

\subsubsection{Layout and separation scheme}
\label{IR.HA.L}
A symmetric final quadrupole doublet layout has been chosen for this design. The beam spot aspect ratio of 2:1 is marginally flatter than the High Luminosity layout, and as such a triplet is less suitable. Figure \ref{fig:IR.HA.L.Layout} and table \ref{tab:IR.HA.L.Layout} detail the layout.\\

\begin{figure*}[!h]
\begin{center}
\includegraphics[scale=0.6]{1_Layout.pdf}
\caption{Layout of machine elements in the High Acceptance IR. Note that the left side of the IR is symmetric.}
\label{fig:IR.HA.L.Layout}
\end{center}
\end{figure*}

\begin{table}[!h]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|}
	\hline
	Element&S$_{entry}$ [m]&L [m]&Gradient [T/m]&Dipole Field [T]&Offset [m]\\ \hline\hline
	BS.L&-21.5&12.7&-&-0.0493&-\\ \hline
	Q2E.L&-8.5&1.0&-77.30906&-0.0493&6.37700$\times 10^{-4}$\\ \hline
	Q1E.L&-7.2&1.0&90.38473&-0.0493&-5.45446$\times 10^{-4}$\\ \hline
	IP&0.0&-&-&-&-\\ \hline
	Q1E.R&6.2&1.0&90.38473&0.0493&5.45446$\times 10^{-4}$\\ \hline
	Q2E.R&7.5&1.0&-77.30906&0.0493&-6.37700$\times 10^{-4}$\\ \hline
	BS.R&8.8&12.7&-&0.0493&-\\ \hline
\end{tabular}
\caption{Machine elements for the High Acceptance IR. S$_{entry}$ gives the leftmost point of the idealised magnetic field of an element. Note that S is relative to the IP.}
\label{tab:IR.HA.L.Layout} 
\end{table}

\noindent The $l$* of 6.2m imposes limitations on focusing and bending in this layout. Focusing is limited by quadratic $\beta$ growth through a drift space, which is increased for smaller $\beta$*. As such, lower instantaneous luminosity is attainable.\\
\\
As in the high luminosity option the beam separation will be achieved by a combination of a adequate crossing angle and the separation fields of off-centre quadrupole magnets. However, due to the large free space of z=6m to the IP, stronger fields have to be applied  to obtain the same geometric separation at the first proton quadrupole. 
\\
Figure \ref{fig:IR.HA.L.Twiss} shows the $\beta$ functions of the beam in both planes from the IP to the face of the final proton quadrupole at s~=~23~m.

\begin{figure*}[!h]
\begin{center}
\includegraphics[scale=0.5]{1_IP_smooth.pdf}
\caption{$\beta$ functions in both planes for the High Acceptance IR layout, from the IP to the face of the final proton quadrupole at s~=~23~m. Note that s is relative to the ring, which begins at the left side of the left dispersion suppressor of IP2.}
\label{fig:IR.HA.L.Twiss}
\end{center}
\end{figure*}


\subsubsection{Optics matching and IR geometry}
\label{IR.HA.LM}
The lattice that is used to match the IR optics to the periodic arc structure corresponds to a large extent to the one presented for the high luminosity option.  Figure \ref{fig:IR.HA.LM.TwissLR} shows the $\beta$ functions of the matching from the IP to the dispersion suppressor, on both sides of the IP (Figure \ref{fig:IR.HA.LM.TwissR}). \\

\begin{table}
\centering
\begin{tabular}{|l|l|l|l|}
	\hline
	Element&S$_{entry}$ [m]&L [m]&Gradient [T/m]\\ \hline
	MQDSF.L2&-268.8944&1.0&9.635332\\ \hline
	MQFM6.L2&-237.5&1.0&-7.436781\\ \hline
	MQDM5.L2&-205.5&1.0&7.676403\\ \hline
	MQFM4.L2&-174.5&1.0&-6.025603\\ \hline
	MQDM3.L2&-143.5&1.0&6.396806\\ \hline
	MQFM2.L2&-111.5&1.0&-9.183061\\ \hline
	MQDM1.L2&-80.5&1.0&5.786843\\ \hline
	MQDM1.R2&79.5&1.0&5.786843\\ \hline
	MQFM2.R2&110.5&1.0&-9.183061\\ \hline
	MQDM3.R2&142.5&1.0&6.396806\\ \hline
	MQFM4.R2&173.5&1.0&-5.894718\\ \hline
	MQDM5.R2&204.5&1.0&7.289766\\ \hline
	MQFM6.R2&236.5&1.0&-7.150586\\ \hline
\end{tabular}
\caption{Machine elements for the High Acceptance LSS layout. S$_{entry}$ gives the leftmost point of the idealised magnetic field of an element. Note that S is relative to the IP.}
\label{tab:IR.HA.LM.Layout}
\end{table}

\begin{figure*}[!h]
%\centering
\begin{center}
\includegraphics[scale=0.5]{1_LSS_smooth.pdf}
\caption{$\beta$ functions in both planes for the High Acceptance IR layout, from the end of the left dispersion suppressor to the start of the right dispersion suppressor. Note that s is relative to the ring, which begins at the left side of the left dispersion suppressor of IP2.}
\label{fig:IR.HA.LM.TwissLR}
\end{center}
\end{figure*}

\begin{figure*}[!h]
%\centering
\begin{center}
\includegraphics[scale=0.5]{1_LSSR_smooth.pdf}
\caption{$\beta$ functions in both planes for the High Luminosity IR layout, from the IP to the start of the right dispersion suppressor. Note that s is relative to the ring, which begins at the left side of the left dispersion suppressor of IP2.}
\label{fig:IR.HA.LM.TwissR}
\end{center}
\end{figure*}

\noindent As with the High Luminosity layout, a smooth matching is obtained, with the IR $\beta$ peaks being brought down and controlled before being matched into the arc solution. The beam envelopes in the LSS are of reasonable size and do not require excessive aperture.\\
\\
Other geometric issues must again be addressed, which are briefly discussed in Section\,\ref{IR.HL.LM}.

\subsection{Comparison of high luminosity and high acceptance options}
\label{IRs.C}
Table \ref{tab:IR.Comp.Params} shows a direct comparison of various parameters of the two layouts.\\

\begin{table}[!h]
\centering
\begin{tabular}{|l|l|l|}
	\hline
	Parameter&HL&HA\\ \hline \hline
	$L(0)$&1.8$\times 10^{33}$&8.54$\times 10^{32}$\\ \hline
	$\theta$&1$\times 10^{-3}$&1$\times 10^{-3}$\\ \hline
	$S(\theta)$&0.746&0.858\\ \hline
	$L(\theta)$&1.34$\times 10^{33}$&7.33$\times 10^{32}$\\ \hline
	$\beta_x*$&0.18 m&0.4 m\\ \hline
	$\beta_y*$&0.1 m&0.2 m\\ \hline
	$\sigma_x*$&3.00$\times 10^{-5}$ m&4.47$\times 10^{-5}$ m\\ \hline
	$\sigma_y*$&1.58$\times 10^{-5}$ m&2.24$\times 10^{-5}$ m\\ \hline
	SR Power&33 kW&51 kW\\ \hline
	$E_c$&126 keV&163 keV\\ \hline
\end{tabular}
\caption{Parameters for the High Luminosity IR.}
\label{tab:IR.Comp.Params}
\end{table}

\noindent The difference in luminosity after considering the loss factor $ \it S $  due to the crossing angle, is a factor of 1.8. However it should be noted that this design strives for technical feasibility and both layouts could be squeezed further to decrease $\beta$* in both planes. The High Luminosity layout could likely be squeezed further than the High Acceptance layout due to the large difference in $l$*, as shown in figure \ref{fig:IR.Comp.Layouts} which compares the two IR layouts. At this stage both designs deliver their required IP parameters of luminosity and acceptance and appear to be feasible.\\
\\
The High Acceptance design generates a  higher level of SR power. This still appears to be within reasonable limits and is discussed in Section\,\ref{NATHAN}. Furthermore, an option is discussed to install a dipole magnet in the detector. This early separation would reduce the required strength of the dipole fields in the IR, significantly reducing total SR power.

\begin{figure*}[!h]
%\centering
\begin{center}
\includegraphics[scale=0.6]{Layout_Comp.pdf}
\caption{Scale comparison of the layouts for the High Luminosity and High Acceptance designs. Note the large difference in $l$*.}
\label{fig:IR.Comp.Layouts}
\end{center}
\end{figure*}


==> machine/newluke.tex <==

\part{Interaction Regions}
\label{IR}
A successful interaction region in an e-p collider must primarily deliver luminosity and detector coverage. Luminosity, both instantaneous and integrated, must be maximised to ensure useful amounts of data are collected. However this should not be pursued at the expense of detector coverage, which is needed to ensure sensitivity to a wide range of processes.

\section{Design Requirements}
\label{IR.Design}
\subsection{Detector Coverage and Acceptance}
\label{IR.Design.MA}
Acceptance describes the amount of angular obstruction of the detector due to the presence of machine elements, as shown in figure \ref{fig:IR.MA.MA}. For example, an acceptance of 10\textdegree~implies a protrusion of machine elements into the detector such that a cone of 10\textdegree~half-angle along the beam axis is blocked. The detector is thus unable to see particles emitted at less than this angle, and event data is lost at high pseudo-rapidities. Note that throughout this section, smaller angles denote higher acceptance.\\

\begin{figure*}[!h]
%\centering
\hspace{-14mm} \includegraphics[scale=0.5]{Acceptance1.pdf}
\caption{Graphical representation of acceptance. $\theta_1$ shows a lower acceptance cone, while $\theta_2$ shows a higher acceptance cone. For machine elements of constant diameter, higher acceptance increases $l$*.}
\label{fig:IR.MA.MA}
\end{figure*}

\noindent Lower acceptance allows machine elements closer to the IP. Since $\beta$ grows quadratically with distance, a smaller $l$* generally allows stronger focusing of a beam and thus higher luminosity. While there is no direct relationship between $l$* and luminosity, a balance must be found to optimise both luminosity and acceptance. Two IR designs are proposed as solutions to the balance between luminosity and acceptance. Both designs aim to achieve a luminosity of $\sim$10$^{33}$~cm$^{-2}$s$^{-1}$.

\begin{enumerate}
\item High Luminosity Layout (HL)
	\begin{itemize}
		\item 10\textdegree~acceptance
		\item Higher luminosity
	\end{itemize}
\item High Acceptance Layout (HA)
	\begin{itemize}
		\item 1\textdegree~acceptance
		\item Lower luminosity
	\end{itemize}
\end{enumerate}

\noindent In concert with these designs, two plans are proposed for running LHeC. One option is to run with the HL layout, then switch to the HA layout during a shutdown. The second option is to optimise the HA layout for sufficient luminosity to replace the HL layout entirely.

\subsection{Beam Separation}
\label{IR.Design.BS}
In an e-p collider IR, there are at least two dissimilar beams. In the case of LHeC, there are two proton beams and an electron beam. One proton beam is brought into collision with the electron beam, while the other, left unsqueezed, is diverted. The unsqueezed beam is addressed in section~\ref{IRs.NCBeam} but from here onward only the squeezed beam is referred to except where explicitly stated.\\
\\
To avoid excessive beam-beam interaction other than at the IP, the beams must be separated quickly. The bunch spacing of 25~ns gives rise to parasitic interaction nodes every 3.75 m before and after the IP. Therefore a separation scheme must be implemented which provides sufficient distance between the beams at these points. A minimum separation of 5$\sigma_e$ + 5$\sigma_p$ is specified at each parasitic node. Beam-beam interactions are discussed in section [ref: Beam-beam section].\\
\\
A further requirement is imposed by the geometry of the IR. An interaction region for an e-p collider involves optics for both the proton and the electron beam. Due to the significantly larger rigidity of the proton beam, the fields used in the proton optics are much stronger than those in the electron optics. While the electron optics do not strongly affect the proton beam, the electron beam will be lost if allowed to pass though the proton optics.\\
\\
However the electron beam emits far more synchrotron radiation for a given bending angle than does the proton beam, and as such the amount by which the electron beam may be deflected inside the IR is limited. Since the electron IR optics are all situated between the IP and the proton IR optics, this constrains the separation which can be obtained by the time the electron beam reaches the proton optics, at s~=~22.96~m.\\
\\
Due to the large proton focusing magnets, it is infeasible to deflect the electron beam sufficiently to complete avoid them. Instead, a half-quadrupole is designed and employed, such that a second aperture with relatively low field may be included for the electron beam to pass through. After this, further bending is applied to the electron beam to extract it back into the electron accelerator ring lattice.\\
\\
Lower fields may be obtained in the electron aperture if the distance between the electron aperture and the proton aperture is increased. Thus separation between the two beams at s~=~22.96~m must still be maximised, whilst not increasing SR power and $\epsilon_c$ to infeasible levels. While this is somewhat flexible, a separation of 55 mm at s~=~23~m has been chosen as an attainable target from optical, radiation [ref:SR section] and magnet design [ref: Magnets section] standpoints.

\subsubsection{Separation Methods}
\label{IR.Design.BS.SM}
The combined requirements of minimising beam-beam interactions and achieving sufficient separation at the proton final quadrupole necessitate the use of multiple separation methods. There are three primary components of the IR separation schemes. Dipoles are used to deflect the electron beam. Due to the limited amount of available space for bending, the electron quadrupoles are offset to induce an additional dipole field, effectively increasing the length of dipole used in the IR. Generally a constant bending radius is used to minimise $\epsilon_c$, although non-constant bends may allow greater control in placement of SR.\\
\\
A crossing angle is also required at the IP to ensure sufficient separation at the first parasitic crossing. However the crossing angle introduces a loss factor in the instantaneous luminosity, given by\\

\begin{equation}
L(\theta) = L_0 S(\theta)
\end{equation}
\label{eqn:LS}

\begin{equation}
S(\theta) = \left[1+\left(\frac{\sigma^2_{sp}+\sigma^2_{se}}{2\sigma^{*2}_x}\right)\tan^2\frac{\theta}{2}\right]^{-\frac{1}{2}}\ .
\label{eqn:S}
\end{equation}\\

\noindent where $\sigma_{sp}$ is the one-sigma width of the proton bunch in the longitudinal direction and $\sigma_{se}$ that of the electron bunch. Beam separation therefore introduces a further optimisation problem with respect to both luminosity and SR. Note the dependence on beam spot size; due to this a more tightly focussed beam will suffer greater losses than a larger beam.

\subsection{Lattice Matching and IR Geometry}
\label{IR.Design.LM}

Once the beams are separated into independent beam pipes, the electron beam must be transported into the ring lattice. Quadrupoles are used in the electron machine LSS to transport the beam from the IP to the dispersion suppressor and match twiss parameters at either end. Space must be available to insert dipoles and further quadrupoles to allow the orbit of the beam to be designed with regard to the physical layout of the ring and the IR.\\
\\
The IR and LSS geometries must be designed around a number of further constraints. As well as beam separation, the electron beam must be steered from the electron ring into the IR and back out again. The colliding proton beam must be largely undisturbed by the electron beam. The non-colliding proton beam must be guided through the IR without interacting with either of the other beams.

\subsection{Proton Beam Matching}
\label{IR.Design.PM}
Parameters at the IP must be such that the existing proton optics may be altered to produce a matched proton beam. Generally an electron beam is flat, with $\epsilon_x$ significantly larger than $\epsilon_y$. However proton beams are generally round, and as such a compromise must be found. In this case, the electron beam's physical cross section is designed to have an aspect ratio of roughly 2:1. The electron beam spot size is also larger than the existing proton beam spot size, and relaxation of the proton optics is simpler than increasing focusing.

\section{High Luminosity IR Layout}
\label{IR.HL}

\subsection{Parameters}
\label{IR.HL.P}
Table \ref{tab:IR.HL.P.Params} details the interaction point parameters and other parameters for this design. To optimise for luminosity, a small $l$* is desired. An acceptance angle of 10\textdegree~is therefore chosen, which gives an $l$* of 1.2m for final focusing quadrupoles of reasonable size.


\begin{table}[!h]
\begin{centering}
\begin{tabular}{|l|l|}
	\hline
	$L(0)$&1.8$\times 10^{33}$\\ \hline
	$\theta$&1$\times 10^{-3}$\\ \hline
	$S(\theta)$&0.746\\ \hline
	$L(\theta)$&1.34$\times 10^{33}$\\ \hline
	$\beta_x*$&0.18 m\\ \hline
	$\beta_y*$&0.1 m\\ \hline
	$\sigma_x*$&3.00$\times 10^{-5}$ m\\ \hline
	$\sigma_y*$&1.58$\times 10^{-5}$ m\\ \hline
	SR Power&33 kW\\ \hline
	$E_c$&126 keV\\ \hline
\end{tabular}
\caption{Parameters for the HL IR.}
\label{tab:IR.HL.P.Params}
\end{centering}
\end{table}

\noindent SR calculations are detailed in section [ref: SR section]. The total power emitted in the IR is similar to that in the HERA-2 IR\cite{HERA2-TDR} and as such appears to be reasonable, given enough space for absorbers.

\subsection{Layout}
\label{IR.HL.L}
A symmetric final quadrupole triplet layout has been chosen for this design, due to the relatively round beam spot aspect ratio of 1.8:1. Figure \ref{fig:IR.HL.L.Layout} and table \ref{tab:IR.HL.L.Layout} detail the layout.\\

\begin{figure*}[!h]
\hspace{-12mm}\includegraphics[scale=0.6]{10_Layout.pdf}
\caption{Layout of machine elements in the HL IR. Note that the left side of the IR is symmetric.}
\label{fig:IR.HL.L.Layout}
\end{figure*}

\begin{table}[!h]
\begin{centering}
\begin{tabular}{|l|l|l|l|l|l|l|}
	\hline
	Element&S$_{entry}$ [m]&L [m]&Gradient [T/m]&Dipole Field [T]&Offset [m]\\ \hline\hline
	BS.L&-21.5&15.8&-&-0.0296&-\\ \hline
	Q3E.L&-5.4&1.0&89.09229&-0.0296&-3.32240$\times 10^{-4}$\\ \hline
	Q2E.L&-4&1.5&-102.2013&-0.0296&2.89624$\times 10^{-4}$\\ \hline
	Q1E.L&-2.2&1.0&54.34071&-0.0296&-5.44711$\times 10^{-4}$\\ \hline
	IP&0.0&-&-&-&-\\ \hline
	Q1E.R&1.2&1.0&54.34071&0.0296&5.44711$\times 10^{-4}$\\ \hline
	Q2E.R&2.5&1.5&-102.2013&0.0296&-2.89624$\times 10^{-4}$\\ \hline
	Q3E.R&4.4&1.0&89.09229&0.0296&3.32240$\times 10^{-4}$\\ \hline
	BS.R&5.7&15.8&-&-0.0296&-\\ \hline
\end{tabular}
\caption{Machine elements for the HL IR. S$_{entry}$ gives the leftmost point of the idealised magnetic field of an element. Note that S is relative to the IP.}
\label{tab:IR.HL.L.Layout} 
\end{centering}
\end{table}


\noindent The $l$* of 1.2 m allows both strong focusing of the beam, and constant bending of the beam from 1.2 m to 21.5 m. This is achieved with offset quadrupoles and a separation dipole.\\
\\
Figure \ref{fig:IR.HL.L.Twiss} shows the $\beta$ functions of the beam in both planes from the IP to the face of the final proton quadrupole at s~=~23~m.

\begin{figure*}[!h]
\hspace{-33mm}\includegraphics[scale=0.6,angle=90]{10_IP_smooth.pdf}
\caption{$\beta$ functions in both planes for the HL IR layout, from the IP to the face of the final proton quadrupole at s~=~23~m. Note that s is relative to the ring, which begins at the left side of the left dispersion suppressor of IP2.}
\label{fig:IR.HL.L.Twiss}
\end{figure*}

\subsection{Separation Scheme}
\label{IR.HL.S}
An FDF electron triplet is used. This has the effect of generating a large peak in $\beta_x$, but is designed such that the peak is between parasitic crossings. The first F quadrupole reduces $\beta_x$ at s~=~3.75~m compared to an initial D quadrupole. The third F quadrupole then brings $\beta_x$ down from the peak sufficiently to avoid large beam-beam interactions at the second parasitic crossing, s~=~7.5~m.\\
\\
This is aided by the bending provided by the offset quadrupoles, and also the IP crossing angle of 1~mrad. These elements ensure that the separation between the beams, normalised to beam size, increases at each parasitic crossing. Note that 1~mrad is not a minimum crossing angle required by beam-beam interaction separation criteria; it is simply a chosen balance between luminosity loss and minimising bend strength. In theory, this layout could support an IP with no crossing angle; however the bend strength required to achieve this would generate an undesirable level of SR power.

\section{High Acceptance IR Layout}
\label{IR.HA}

\subsection{Parameters}
\label{IR.HA.P}
Table \ref{tab:IR.HA.P.Params} details the interaction point parameters and other parameters for this design. The chosen acceptance for this layout is 1\textdegree. For final electron focusing magnets of reasonable strength this places all elements outside the limits of the detector, at z~=~±6.2m, where z the is longitudinal axis of the detector. Due to the small crossing angle the magnets are thus placed at s~=~±6.2m. As such, the actual acceptance of the layout is limited by the beam pipe rather than the size of machine elements. This also gives further flexibility in the strengths and designs of the final focusing quadrupoles, although this flexibility is not exploited in the design.\\

\begin{table}[!h]
\centering
\begin{tabular}{|l|l|}
	\hline
	$L(0)$&8.54$\times 10^{32}$\\ \hline
	$\theta$&1$\times 10^{-3}$\\ \hline
	$S(\theta)$&0.858\\ \hline
	$L(\theta)$&7.33$\times 10^{32}$\\ \hline
	$\beta_x*$&0.4 m\\ \hline
	$\beta_y*$&0.2 m\\ \hline
	$\sigma_x*$&4.47$\times 10^{-5}$ m\\ \hline
	$\sigma_y*$&2.24$\times 10^{-5}$ m\\ \hline
	SR Power&51 kW\\ \hline
	$E_c$&163 keV\\ \hline
\end{tabular}
\caption{Parameters for the HA IR.}
\label{tab:IR.HA.P.Params}
\end{table}

\noindent SR calculations are detailed in section [ref: SR section]. The total power emitted in the IR is similar to that in the HERA-2 IR\cite{HERA2-TDR} and as such appears to be reasonable, given enough space for absorbers. However it is significantly higher than that in the HL layout. As discussed in section [ref: SR section], an option exists to reduce the total SR power by including a dipole field in the detector, thus mitigating the limitation imposed on dipole length by the larger $l$*.

\subsection{Layout}
\label{IR.HA.L}
A symmetric final quadrupole doublet layout has been chosen for this design. The beam spot aspect ratio of 2:1 is marginally flatter than the HL layout, and as such a triplet is less suitable. Figure \ref{fig:IR.HA.L.Layout} and table \ref{tab:IR.HA.L.Layout} detail the layout.\\

\begin{figure*}[!h]
\hspace{-12mm}\includegraphics[scale=0.6]{1_Layout.pdf}
\caption{Layout of machine elements in the HA IR. Note that the left side of the IR is symmetric.}
\label{fig:IR.HA.L.Layout}
\end{figure*}

\begin{table}[!h]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|}
	\hline
	Element&S$_{entry}$ [m]&L [m]&Gradient [T/m]&Dipole Field [T]&Offset [m]\\ \hline\hline
	BS.L&-21.5&12.7&-&-0.0493&-\\ \hline
	Q2E.L&-8.5&1.0&-77.30906&-0.0493&6.37700$\times 10^{-4}$\\ \hline
	Q1E.L&-7.2&1.0&90.38473&-0.0493&-5.45446$\times 10^{-4}$\\ \hline
	IP&0.0&-&-&-&-\\ \hline
	Q1E.R&6.2&1.0&90.38473&0.0493&5.45446$\times 10^{-4}$\\ \hline
	Q2E.R&7.5&1.0&-77.30906&0.0493&-6.37700$\times 10^{-4}$\\ \hline
	BS.R&8.8&12.7&-&0.0493&-\\ \hline
\end{tabular}
\caption{Machine elements for the HA IR. S$_{entry}$ gives the leftmost point of the idealised magnetic field of an element. Note that S is relative to the IP.}
\label{tab:IR.HA.L.Layout} 
\end{table}

\noindent The $l$* of 6.2m imposes limitations on focusing and bending in this layout. Focusing is limited by quadratic $\beta$ growth through a drift space, which is increased for smaller $\beta$*. As such, lower instantaneous luminosity is attainable.\\
\\
Although offset quadrupoles are used to separate the beams, this layout has less total dipole length available. Additionally, the first parasitic crossing occurs before the beam is focused in the first quadrupole. This further limits final focusing as the beam cannot be permitted to grow too large by this time. The loss of dipole length also means stronger bending must be used later, increasing SR power generation.\\
\\
Figure \ref{fig:IR.HA.L.Twiss} shows the $\beta$ functions of the beam in both planes from the IP to the face of the final proton quadrupole at s~=~23~m.

\begin{figure*}[!h]
\hspace{-33mm}\includegraphics[scale=0.6,angle=90]{1_IP_smooth.pdf}
\caption{$\beta$ functions in both planes for the HA IR layout, from the IP to the face of the final proton quadrupole at s~=~23~m. Note that s is relative to the ring, which begins at the left side of the left dispersion suppressor of IP2.}
\label{fig:IR.HA.L.Twiss}
\end{figure*}

\subsection{Separation Scheme}
\label{IR.HA.S}
The final electron doublet is arranged such that the peak in $\beta_y$ is large, while the peak in $\beta_x$ is controlled and kept small. Unlike the HL layout, the first parasitic crossing is reached before focusing begins. As such there is a minimum crossing angle of roughly 0.7~mrad, which is dependent solely upon $\beta$ growth in the drift space. For comparison with the HL layout, and as a balance between luminosity loss and SR power generation, a crossing angle of 1~mrad has been chosen.

\section{Comparison of Layouts}
\label{IRs.C}
Table \ref{tab:IR.Comp.Params} shows a direct comparison of various parameters of the two layouts.\\

\begin{table}[!h]
\centering
\begin{tabular}{|l|l|l|}
	\hline
	Parameter&HL&HA\\ \hline \hline
	$L(0)$&1.8$\times 10^{33}$&8.54$\times 10^{32}$\\ \hline
	$\theta$&1$\times 10^{-3}$&1$\times 10^{-3}$\\ \hline
	$S(\theta)$&0.746&0.858\\ \hline
	$L(\theta)$&1.34$\times 10^{33}$&7.33$\times 10^{32}$\\ \hline
	$\beta_x*$&0.18 m&0.4 m\\ \hline
	$\beta_y*$&0.1 m&0.2 m\\ \hline
	$\sigma_x*$&3.00$\times 10^{-5}$ m&4.47$\times 10^{-5}$ m\\ \hline
	$\sigma_y*$&1.58$\times 10^{-5}$ m&2.24$\times 10^{-5}$ m\\ \hline
	SR Power&33 kW&51 kW\\ \hline
	$E_c$&126 keV&163 keV\\ \hline
\end{tabular}
\caption{Parameters for the HL IR.}
\label{tab:IR.Comp.Params}
\end{table}

\noindent The difference in luminosity after considering losses due to the crossing angle is a factor of 1.8. However it should be noted that this design strives for technical feasibility and both layouts could potentially be squeezed further to decrease $\beta$* in both planes. The HL layout could likely be squeezed further than the HA layout due to the large difference in $l$*, as shown in figure \ref{fig:IR.Comp.Layouts} which compares the two IR layouts. At this stage both designs deliver their required IP parameters of luminosity and acceptance and appear feasible.\\
\\
The HA design generates more SR power. This appears to be within reasonable limits and is discussed in section [ref: SR section]. Furthermore, an option is discussed to install a dipole magnet in the detector. This early separation would reduce the required strength of the dipole fields in the IR, significantly reducing total SR power. However this option is challenging and is unlikely to be required.

\begin{figure*}[!h]
%\centering
\hspace{-12mm}\includegraphics[scale=0.6]{Layout_Comp.pdf}
\caption{Scale comparison of the layouts for the HL and HA designs. Note the large difference in $l$*.}
\label{fig:IR.Comp.Layouts}
\end{figure*}

\section{Long Straight Section}
\label{IRs.LSS}
The Long Straight Section (LSS) geometrically and optically matches the IR to the rest of the LHeC ring lattice. For the purposes of this report, the LSS is defined from the start of the left dispersion suppressor (DS) to the end of the right DS. This is due to the need to alter the DS's optically and geometrically from the nominal design to obtain a solution.\\
\\
The LSS geometry uses a complex bending scheme in the horizontal and vertical planes to satisfy the various constraints. These include the 0.6~m radial offset of the LHeC ring as mentioned in section~[ref: Ring lattice section], the 1~m vertical offset, and the IR separation geometry. This results in a small path length difference which must be compensated elsewhere in the ring, nominally in the bypasses. Since the LSS design iterates relatively frequently these changes have not been made in the LHeC lattice, but do not present a challenge. Due to the large amount of bending required, SR generation is also a constraint.\\
\\
It should be noted that in the current LSS design there are some conflicts between LHeC LSS magnet placements and LHC LSS magnet placements. The aim has been to design a self-consistent LHeC solution, and then iterate upon this to eliminate these conflicts. Future plans are discussed later in this section. It should also be noted that the solution presented is only matched for the HA IR layout. However generating a similar solution for the HL layout presents no additional challenges.

\subsection{Dispersion}
\label{IRs.LSS.D}
A key constraint coupled to optics and geometry is dispersion. Since dispersion is an optical quantity generated by geometry, this becomes a challenge for the complex LSS bending scheme. The LHeC DSs are designed to match horizontal dispersion from the LSS to the arc. There is no equivalent scheme to deal with large vertical dispersion. Therefore an achromatic vertical separation scheme is used. Two vertical double bend achromat (DBA) sections on either side of the IR form doglegs while generating no vertical dispersion. This complicates optical matching due to limited optical flexibility of the DBA scheme. Figures~\ref{fig:IR.LSS.D.DBAGeom} and \ref{fig:IR.LSS.D.DBAOptics} detail the geometry and optics of the DBA sections used in the LSS.

\begin{figure*}[!h]
\hspace{-30mm}\includegraphics[scale=0.6]{DBAGeom.pdf}
\caption{Geometry plot for a DBA dogleg pair in the HA LSS design.}
\label{fig:IR.LSS.D.DBAGeom}
\end{figure*}

\begin{figure*}[!h]
\hspace{-30mm}\includegraphics[scale=0.6]{DBAOptics.pdf}
\caption{Optics plot for a single DBA module in the HA LSS design. Note waists and peaks in $\beta_y$.}
\label{fig:IR.LSS.D.DBAOptics}
\end{figure*}

\subsection{Geometry}
\label{IRs.LSS.Geom}
Figure~\ref{fig:IR.LSS.Geom.LSSGeom} shows the geometry of the LSS solution. Note that the vertical doglegs are placed between the two horizontal dipole sets. To maximise use of space, schemes were explored with interleaved horizontal and vertical bends, as shown in figure~\ref{fig:IR.LSS.Geom.LSSCoupled}. This allows increased bend length and distance between bends, reducing SR generation. However this coupled bending generates rotation of the beam around the s axis, effectively causing all subsequent quadrupoles to have a skew component.\\

\begin{figure*}[!h]
\hspace{-30mm}\includegraphics[scale=0.6]{LSSSurvey.pdf}
\caption{Geometry of the LSS design. Due to small angles involved, the s axis approximates the z axis well, and is used to allow MADX to display lattice elements.}
\label{fig:IR.LSS.Geom.LSSGeom}
\end{figure*}

\begin{figure*}[!h]
\hspace{-30mm}\includegraphics[scale=0.6]{Roll.pdf}
\caption{Example of geometry of a design with coupled horizontal and vertical bends. Interleaving bends in this way generates roll around s axis. The IP is at zero in both axes.}
\label{fig:IR.LSS.Geom.LSSCoupled}
\end{figure*}

\noindent Note that the left DS has nominal bend strength, while the right DS dipoles are weakened to accommodate the 1.2~m horizontal separation. Note also that future iterations of the LSS will include changes to accommodate the solution for the non-colliding proton beam detailed in section~\ref{IRs.NCBeam}. In practise this simply manifests as a rotation of the IR section, and no complex changes are required.

\subsection{Optics}
\label{IRs.LSS.Optics}
Placement of quadrupole elements is constrained by LSS geometry requirements, and by LHC element placement, although this constraint is ignored for this iteration. While the LSS horizontal dipoles alone do not significantly constrain space, the combination of these and the vertical DBA takes up large amounts of space. Importantly, the vertical DBAs are long and cannot be interrupted with extra quadrupoles since quadrupoles are used to satisfy the achromatic condition.\\
\\
Quadrupole triplets are used in the centre of the DBAs to allow some matching flexibility. A single quadrupole would have a fixed strength to cancel dispersion. The triplet DBA still generates a characteristic beta function shape, resulting in peaks and waists which make matching more challenging. Figure~\ref{fig:IR.LSS.Optics.Optics} shows the beta and dispersion functions of the LSS optics. Matching is feasible but the solution is complex.

\begin{figure*}[!h]
\hspace{-30mm}\includegraphics[scale=0.6]{LSSOptics.pdf}
\caption{Optics plot for the HA LSS design.}
\label{fig:IR.LSS.Optics.Optics}
\end{figure*}

\subsection{Synchrotron Radiation}
\label{IRs.LSS.SR}
While detailed simulations have not yet been run, a simple analytical calculation of SR generated by the dipoles in the LSS has been performed, giving an initial estimate of $\sim$1.4~MW. Note that this includes the left and right DS sections. This is manageable considering the $\sim$50~MW estimate for the rest of the ring.

\subsection{LHC Integration}
\label{IRs.LSS.LHC}
Currently, the DBA modules and quadrupoles near the IP conflict with the LHC proton triplet. After sufficient horizontal and/or vertical separation electron elements may be placed arbitrarily. Plans for future iterations to resolve conflicts include moving vertical separation outward from the IP, after horizontal separation. In this case, no quadrupoles are required until $\sim$80~m from the IP, leaving space for the proton triplet.\\
\\
This scheme would change optical constraints. In the current "early" vertical separation scheme, limited space between the IR and the DBA decreases matching flexibility. In a "late" vertical separation design, flexibility between the IR and DBA increases, but decreases correspondingly between the DBA and the DS.\\
\\
Note that it is to some degree possible to reduce a bending scheme's space requirements arbitrarily, at the cost of more SR power.

\section{Non-Colliding Proton Beam}
\label{IRs.NCBeam}
In both IRs, a solution must be found for dealing with the second proton beam. The second beam must not collide with either of the other two beams, or generate significant beam-beam effects. Also, detector designs strongly prefer for the second beam to occupy the same central beam pipe as the other two beams, rather than allowing space through the detector for a second pipe.

\subsection{Design Elements}
\label{IRs.NCBeam.Design}
To avoid collisions and beam-beam effects, the bunches of the non-colliding (NC) beam are offset in time. This prevents proton-proton collisions at the IP, and allows the NC beam to overlap with the co-rotating electron beam.\\
\\
Proton-proton parasitic interactions and beam-beam effects can still occur. To minimise these, the NC beam is left unsqueezed, and a proton-proton crossing angle is implemented. The unsqueezed beam minimises effective luminosity at parasitic crossings, and the crossing angle generates separation. For unsqueezed optics, LHC alignment optics [CDR v1.0 reference 664] are modified for use on the NC beam only. The optics used is the same as in the linac-ring design in section [LR IR].\\
\\
A crossing angle is generated by changing the LHC separator dipoles D1 and D2. Figure~\ref{fig:IR.NCBeam.Design.3Beam} shows the trajectories of the three beams for the HA design. The proton final triplet is rotated and moved to match the new trajectory of the colliding beam. Its position in s stays constant.\\

\begin{figure*}[!h]
\hspace{-5mm}\includegraphics[scale=0.5]{NC_3BeamPlot.pdf}
\caption{Trajectories of the three beams in the HA interaction region design. Note that in this plot the beams are reversed compared to the LSS plots.}
\label{fig:IR.NCBeam.Design.3Beam}
\end{figure*}

\noindent Note that the electron trajectory is rotated to match the colliding proton beam, such that the electron-proton crossing angle is still 1~mrad. This requires a change to the LSS geometry and optics solution which has not yet been implemented. This will be included in the next iteration of the LSS design. No new issues are likely to be introduced. Note also that the electron IR itself is unchanged in both the HL and HA designs, so SR calculations and detector designs do not require updates.

\subsection{Solution}
\label{IRs.NCBeam.Soltn}
For unsqueezed optics, zero triplet strength is required for the NC beam. The triplet quadrupoles each have a single proton aperture and as such the proton beams cannot be focused differently if both pass through the main aperture. Therefore the NC beam is guided through the same aperture as the electron beam, and experiences effectively no focusing. The proton LSS matching quadrupoles, which are separately powered for each beam, are then used to implement the NC beam optics.\\
\\
As shown in section [ref: Magnets section], Q1 will be a half-quadrupole. A large field-free aperture accomodates the electron beam and the NC proton beam. Q2 and Q3 have standard designs which incorporate low-field pockets. These holes will be used for the shared electron and NC proton apertures.\\
\\
Aperture calculations are based on 15$\sigma$ proton envelopes and 20$\sigma$ electron envelopes. In both IRs, aperture is driven by horizontal requirements, since the horizontal envelopes and horizontal separation dominate over the vertical electron envelope. Note that the Q2 and Q3 apertures are circular; aperture radius is thus determined by the larger dimension.

\subsubsection{High Luminosity}
\label{IRs.NCBeam.Soltn.HA}
The proton-proton crossing angle is optimised to 3~mrad to minimise aperture requirements, by making the NC beam follow the electron beam closely. The electron trajectory is determined by the IR separation scheme. It is impossible to have the proton beam exactly follow the electron beam due to the offset between the two generated by the separation scheme. The electron beam, having larger emittance, dominates aperture requirements. Table~\ref{tab:IR.NCBeam.Soltn.HL.Apertures} and figure~\ref{fig:IR.NCBeam.Soltn.HL.Apertures} show the required apertures.

\begin{table}[!h]
\centering
\begin{tabular}{|l|l|l|}
\hline
Element&Ap Radius&Ap Centre\\
\hline
Q1&0.0311&-0.0666\\
\hline
Q2A&0.0274&-0.1001\\
\hline
Q2B&0.0259&-0.1251\\
\hline
Q3&0.0257&-0.1592\\
\hline
\end{tabular}
\caption{Proton triplet aperture requirements for the HL layout.}
\label{tab:IR.NCBeam.Soltn.HL.Apertures}
\end{table}

\begin{figure*}[!h]
\hspace{-15mm}\includegraphics[scale=0.5]{NC_ApertureHL.pdf}
\caption{Proton triplet aperture requirements with trajectories and envelopes of the electron beam and NC proton beam for the HL layout. Note that in this plot the beams are reversed compared to the LSS plots.}
\label{fig:IR.NCBeam.Soltn.HL.Apertures}
\end{figure*}

\subsubsection{High Acceptance}
\label{IRs.NCBeam.Soltn.HA}
The proton-proton crossing angle is optimised to 3.4~mrad to minimise aperture requirements, by making the NC beam follow the electron beam closely. The electron trajectory is determined by the IR separation scheme. The electron beam, having larger emittance, dominates aperture requirements. The separation between the electron beam and the NC proton beam is larger in the HA layout than in the HL layout, due to the later bending in the HA separation scheme. This increases aperture requirements. Table~\ref{tab:IR.NCBeam.Soltn.HA.Apertures} and figure~\ref{fig:IR.NCBeam.Soltn.HA.Apertures} show the required apertures.

\begin{table}[!h]
\centering
\begin{tabular}{|l|l|l|}
\hline
Element&Aperture Radius&Aperture Centre\\
\hline
Q1&0.0296&-0.0752\\
\hline
Q2A&0.0227&-0.1100\\
\hline
Q2B&0.0233&-0.1402\\
\hline
Q3&0.0264&-0.1811\\
\hline
\end{tabular}
\caption{Proton triplet aperture requirements for the HA layout.}
\label{tab:IR.NCBeam.Soltn.HA.Apertures}
\end{table}

\begin{figure*}[!h]
\hspace{-15mm}\includegraphics[scale=0.5]{NC_ApertureHA.pdf}
\caption{Proton triplet aperture requirements with trajectories and envelopes of the electron beam and NC proton beam for the HA layout. Note that in this plot the beams are reversed compared to the LSS plots.}
\label{fig:IR.NCBeam.Soltn.HA.Apertures}
\end{figure*}

\subsection{Summary}
\label{IRs.NCBeam.Summary}

Aperture requirements for the HL layout are somewhat less demanding than for the HA layout, but both sets of requirements are feasible and do not present difficulties in magnet design using existing technology. The existing Q1 design is easily sufficient. Q2A and Q2B would ideally be two copies of the same yoke, requiring a larger hole in each. Q3 requires a larger yoke than the existing 200~mm radius design, but the tooling limit of 270~mm should be sufficient.\\
\\
In both designs, the crossing angle may be increased if desired for beam-beam reasons. The existing Q1 design supports a crossing angle up to 4~mrad, but this would require significantly larger apertures in the other magnets.



==> machine/rinolfi.tex <==
\section{Positron options for the Linac-Ring option}

Figure $\ref{Fig:LHeCInjector5}$ shows the layout of the LPI (LEP Pre-Injector) as it was
working in 2000.

LPI was composed of the LIL (LEP Injector Linac) and the EPA (Electron
Positron Accumulator).


\begin{figure}
\begin{center}
\includegraphics[width=0.8\columnwidth]{LHeCInjector_Fig5}
\caption{Layout of the LPI in 2000.}
\label{Fig:LHeCInjector5}
\end{center}
\end{figure} 

Table $\ref{tab:rinolfi6}$ gives the beam characteristics at the end of LIL.

\begin{table}[h]
\centering
\begin{tabular}{|l|l|}
\hline
Beam energy & $200$ to $700$ MeV \\ \hline
Charge & $5 \times 10^8$ to $2 \times 10^{10} e^-$ / pulse \\ \hline
Pulse length & $10$ to $40$ ns (FWHM) \\ \hline
Repetition frequency & $1$ to $100$ Hz \\ \hline
Beam sizes (rms) & $3$ mm \\ \hline
\end{tabular}
\caption{LIL beam parameters.}
\label{tab:rinolfi6}
\end{table}



Figure $\ref{Fig:LHeCInjector6}$ shows an electron beam profile at the end of LIL (500 MeV).

\begin{figure}
\begin{center}
\includegraphics[width=0.8\columnwidth]{LHeCInjector_Fig6}
\caption{Electron beam profile at 500 MeV.}
\label{Fig:LHeCInjector6}
\end{center}
\end{figure} 

Table $\ref{tab:rinolfi7}$ gives the electron and positron beam parameters at the exit of EPA.

\begin{table}[h]
\centering
\begin{tabular}{|l|l|}
\hline
Energy & $200$ to $600$ MeV \\ \hline
Charge & up to $4.5 \times 10^{11} e{\pm}$ \\ \hline
Intensity & up to $0.172$ A \\ \hline
Number of buckets & $1$ to $8$ \\ \hline
Emittance & $0.1$ mm.mrad \\ \hline
Tune & $Q_x = 4.537, Q_y = 4.298$ \\ \hline
\end{tabular}
\caption{The electron and positron beam parameters at the exit of EPA.}
\label{tab:rinolfi7}
\end{table}

In summary, the LPI characteristics fulfil completely the
requested performance for the LHeC injector based on Ring-Ring
option.



==> machine/rinolfirr.tex <==

\section{LHeC injector for the Ring-Ring option}

Figure $\ref{Fig:LHeCInjector5}$ shows the layout of the LPI (LEP Pre-Injector) as it was
working in 2000.

LPI was composed of the LIL (LEP Injector Linac) and the EPA (Electron
Positron Accumulator).


\begin{figure}
\begin{center}
\includegraphics[width=0.8\columnwidth]{LHeCInjector_Fig5}
\caption{Layout of the LPI in 2000.}
\label{Fig:LHeCInjector5}
\end{center}
\end{figure} 

Table $\ref{tab:rinolfi6}$ gives the beam characteristics at the end of LIL.

\begin{table}[h]
\centering
\begin{tabular}{|l|l|}
\hline
Beam energy & $200$ to $700$ MeV \\ \hline
Charge & $5 \times 10^8$ to $2 \times 10^{10} e^-$ / pulse \\ \hline
Pulse length & $10$ to $40$ ns (FWHM) \\ \hline
Repetition frequency & $1$ to $100$ Hz \\ \hline
Beam sizes (rms) & $3$ mm \\ \hline
\end{tabular}
\caption{LIL beam parameters.}
\label{tab:rinolfi6}
\end{table}



Figure $\ref{Fig:LHeCInjector6}$ shows an electron beam profile at the end of LIL (500 MeV).

\begin{figure}
\begin{center}
\includegraphics[width=0.8\columnwidth]{LHeCInjector_Fig6}
\caption{Electron beam profile at 500 MeV.}
\label{Fig:LHeCInjector6}
\end{center}
\end{figure} 

Table $\ref{tab:rinolfi7}$ gives the electron and positron beam parameters at the exit of EPA.

\begin{table}[h]
\centering
\begin{tabular}{|l|l|}
\hline
Energy & $200$ to $600$ MeV \\ \hline
Charge & up to $4.5 \times 10^{11} e{\pm}$ \\ \hline
Intensity & up to $0.172$ A \\ \hline
Number of buckets & $1$ to $8$ \\ \hline
Emittance & $0.1$ mm.mrad \\ \hline
Tune & $Q_x = 4.537, Q_y = 4.298$ \\ \hline
\end{tabular}
\caption{The electron and positron beam parameters at the exit of EPA.}
\label{tab:rinolfi7}
\end{table}

In summary, the LPI characteristics fulfils completely the
requested performance for the LHeC injector based on Ring-Ring
option.



==> physics/bsm_bib.tex <==

% -- Contact Interactions

% form factor
\bibitem{koepp} G.~K\"opp, D.~Schaile, M.~Spira and P.M.~Zerwas,
                Z.~Phys. C~65 (1995) 545.

\bibitem{kinoshita} see reviews by T.~Kinoshita and D.R.~Yennie,
  H.-U.~Martyn, and R.S.~van~Dyck~Jr. in {\em `Quantum Electrodynamics`},
  ed. T.~Kinoshita, World Scientific (1990).

% CI phenomenology
\bibitem{elpr} E.J.~Eichten, K.D.~Lane and M.E.~Peskin,
               Phys. Rev. Lett. 50 (1983) 811; \\
               R.~R\"uckl, Phys. Lett. B~129 (1983) 363 and
               Nucl. Phys. B~234 (1984) 91.

\bibitem{haberl} P.~Haberl, F.~Schrempp and H.-U.~Martyn,
                 Proc. Workshop {\em `Physics at HERA'},
                 eds. W.~Buchm\"uller and G.~Ingelman,
                 DESY, Hamburg (1991), vol. 2, p. 1133.

\bibitem{Zarnecki} A.F.~Zarnecki, Eur. Phys. J. {\bf C11} 539 (1999) [hep-ph/9904334].


% -- Leptoquarks

\bibitem{BRW}
 W.~Buchm\"uller, R.~R\"uckl and D.~Wyler, Phys.~Lett.~B191 (1987) 442.
{\it{Erratum}} Phys.~Lett.~B448 (1999) 320.

\bibitem{AACHEN}
 B.~Schrempp, Proc. of the Workshop ``Physics at HERA",
 DESY, Hamburg (1991), vol. 2 p. 1034, {\it and references therein},
 W.~Buchm\"uller and G.~Ingelman (Editors).
%
\bibitem{DAVIDSON}
S.~Davidson, D.~Bailey and B.~Campbell, Z. Phys. C61 (1994) 613.
%
\bibitem{LEURER}
M.~Leurer, Phys. Rev. D49 (1994) 333; {\it idem.} D50 (1994) 536.
%
\bibitem{RIZZO}
 J.L.~Hewett and T.G.~Rizzo,
 Phys. Rev. D58:055005 (1998).
%

\bibitem{filip}
A.F.~Zarnecki, proceedings of DIS08.

\bibitem{belaev}
  A.~Belyaev, C.~Leroy, R.~Mehdiyev and A.~Pukhov,
  %``Leptoquark single and pair production at LHC with calcHEP/compHEP in  the
  %complete model,''
  JHEP {\bf 0509} (2005) 005 [hep-ph/0502067].
%

\bibitem{peterz}
J.~Ohnemus, S.~Rudaz, T.~F.~Walsh and P.~M.~Zerwas,
  %``Single leptoquark production at hadron colliders,''
  Phys.\ Lett.\ B {\bf 334} (1994) 203
  [hep-ph/9406235].
%



% -- Excited fermions

\bibitem{Harari:1982xy}
  H.~Harari,
%  ``Composite Models For Quarks And Leptons,''
  Phys.\ Rept.\  {\bf 104} (1984) 159.

\bibitem{LHCExcitedLepton} O.~J.~Eboli, S.~M.~Lietti and P.~Mathews, Phys.~Rev.~{\bf D 65} (2002) 075003.
\bibitem{NLCExcitedLepton} E.~M.~Gregores, M.~C.~Gonzalez-Garcia, and S.~F.~Novaes, Phys.~Rev.~{\bf D 56} (1997) 2920.

\bibitem{ExcitedElectronPaper}F. D. Aaron {\it et al.} [H1 Collaboration], \Journal{\PLB}{666}{131}{2008} [hep-ex/08054530].

\bibitem{ExcitedNeutrinoPaper}F. D. Aaron {\it et al.} [H1 Collaboration], \Journal{\PLB}{663}{382}{2008} [hep-ex/08021858].


\bibitem{ExcitedQuarkPaper} F. D. Aaron {\it et al.} [H1 Collaboration], \Journal{\PLB}{678}{335}{2009} [hep-ex/09043392].


\bibitem{ExcitedElectronPaperOPAL}G. Abbiendi {\it et al.} [OPAL Collaboration], \Journal{\PLB}{544}{57}{2002} [hep-ex/0206061].

\bibitem{ExcitedElectronPaperDELPHI}J. Abdallah  {\it et al.} [DELPHI Collaboration], \Journal{\EPJC}{37}{405}{2004} [hep-ex/0409058].

\bibitem{ExcitedElectronPaperCDF}D. Acosta  {\it et al.} [DO Collaboration], \Journal{\PRD}{77}{091102}{2008} [hep-ex/08010877].

\bibitem{CompositnessModel1}K. Hagiwara, D. Zeppenfeld and S. Komamiya, \Journal{\ZPC}{29}{115}{1985}.

\bibitem{CompositnessModel2}F. Boudjema, A. Djouadi and J. L. Kneur, \Journal{\ZPC}{57}{425}{1993}.

\bibitem{CompositnessModel3}U. Baur, M. Spira and P. M. Zerwas, \Journal{\PRD}{42}{815}{1990}.
 \bibitem{GeneratorCOMPOS} T. Kohler, Proceeding of the Workshop "Physics at HERA", eds. W. Buchmuller and G. Ingelman, DESY (1991), Vol 3, p 1526.

\bibitem{SpiraPrivateCom}M. Spira, private communication.
 \bibitem{GeneratorWabgen}C. Berger and P. Kandel, "A New Generator For Wide Angle Bremsstrahlung", Proceedings of the Workshop "Monte Carlo Generators for HERA Physics", eds. A. T. Doyle, G. Grindhammer, G. Ingelman and H. Jung, DESY (1998).




% --- 4th family


\bibitem{Arik98}E. Arik et al., Phys. Rev. D \textbf{58}, 117701
(1998); I.F. Ginzburg, I.P. Ivanov, A. Schiller, Phys. Rev. D \textbf{60},
095001 (1999); B. Holdom, JHEP \textbf{0608}, 076 (2006); G. D. Kribs,
T. Plehn, M. Spannowsky and T. M. P. Tait, Phys. Rev. D \textbf{76},
075016 (2007); V. E. Ozcan, S. Sultansoy and G. Unel, Eur. Phys. J.
C \textbf{57} , 621 (2008); O. Cakir, H. Duran Yildiz, R. Mehdiyev
and I. Turk Cakir, Eur. Phys. J. C \textbf{56}, 537 (2008); R. Ciftci,
Phys. Rev. D \textbf{78}, 075018 (2008); E.V. Ozcan, S. Sultansoy,
G. Unel, J. Phys. G \textbf{36}, 095002 (2009); I.T. Cakir et al.,
Phys. Rev. D \textbf{80}, 095009 (2009).

\bibitem[2]{Erler10} J. Erler, P. Langacker, arXiv:1003.3211v2 {[}hep-ph].

\bibitem[3]{Maltoni00} M. Maltoni \emph{et al.}, Phys. Lett. B \textbf{476},
107 (2000); V.A. Novikov, A.N. Rozanov, M.I. Vysotsky, arXiv:0904.4570
{[}hep-ph].

\bibitem[4]{CDF10-1} J. Conway et al., CDF Collaboration, CDF Note
10110.

\bibitem[5]{CDF10} T. Aaltonen et al., CDF Collaboration, arXiv:0912.1057
{[}hep-ex].

\bibitem[6]{Amsler08} C. Amsler \textit{et al.}, {[}Particle Data
Group], Phys. Lett. B \textbf{667}, 1 (2008); P. Achard \textit{et
al.}, {[}L3 Collaboration], Phys. Lett. B \textbf{517}, 75 (2001).

\bibitem[7]{Cakir09} O. Cakir, A. Senol and A. T. Tasci, Eur. Phys.
Lett. \textbf{88}, 11002 (2009); O.Cakir, V. Cetinkaya, arXiv:0912.2041
{[}hep-ph].

\bibitem[8]{Pukhov99} A.Pukhov \emph{et al}., arXiv:hep-ph/9908288;
E.Boos \emph{et al.} {[}CompHEP Collaboration], Nucl. Instrum. Meth.
A \textbf{534}, 250 (2004) (arXiv:hep-ph/0403113).

\bibitem[9]{Pumplin07} J. Pumplin \emph{et al.}, JHEP \textbf{0207},
012 (2002), arXiv:hep-ph/0201195.

\bibitem[10]{Hou07} W.S. Hou, M. Nagashima, a. Soddu, Phys. Rev.
D \textbf{76}, 016004 (2007); M.S. Chanowitz, Phys. Rev. D \textbf{79},
113008 (2009); M.~Bobrowski, A.~Lenz, J.~Riedl and J.~Rohrwild,
Phys. Rev. D \textbf{79}, 113006 (2009).

\bibitem[11]{Ozcan08}V. E. Ozcan, S. Sultansoy and G. Unel, Eur.
Phys. J. C \textbf{57} , 621 (2008).






==> physics/bsm_ciftci_fourth.tex <==
\newpage
\subsection{Production of the fourth SM family fermions at the Large Hadron
  electron Collider}

\vspace{0.2cm}
\noindent
A.Kenan Çiftçi, Rena Çiftçi and Saleh Sultansoy ~~~~~~ Ankara U., Ankara U. and TOBB ETU 10.08.2010
%------------------------------------
%
% Start of the text proper
%


Ref. \cite{Fritzsch:1999rd} reasons that t-quark anomalous interactions may exist due to its large mass. With similar arguments, one can show that anomalous interactions appear to be quite natural for the fourth generation fermions.  The discovery capacity of lepton collider could be enlarged if the anomalous interactions of the fourth generation fermions with the first three ones exist.  These anomalous interactions could provide also single production of the fourth generation fermions at future lepton-hadron \cite{Ciftci:2007rv,Ciftci:2006fw} and gamma-hadron colliders.
The effective Lagrangian for magnetic type anomalous interaction of the fourth generation charged lepton and neutrino are
\begin{itemize} 	
  \item {${\cal L}_{nc}=\left(\frac{\kappa^{\ell_4\ell_{i}}_\gamma}{\Lambda}\right)e_{\ell}g_{e}\overline{\ell_{4}}\sigma_{\mu\nu}\ell_{i}F^{\mu\nu}+\left(\frac{\kappa^{\ell_4\ell_{i}}_Z}{2\Lambda}\right)g_{Z}\overline{\ell_{4}}\sigma_{\mu\nu}\ell_{i}Z^{\mu\nu}+h.c. $}
	\item ${\cal L}_{cc}=\left(\frac{g_{W} }{\sqrt{2}}\right)\overline{l_{i}}\left[\left|V_{\nu_4l_{i}}\right|\gamma_\mu+\frac{i}{2 \Lambda}\kappa^{\nu_{4}l_{i}}_{W}\sigma_{\mu\nu}q^{\nu}\right]P_L\nu_{4}W^{\mu}+h.c.$
	\item ${\cal L}_{nc}=\left(\frac{g_{Z}}{2}\right)\overline{\nu_{i}}\frac{i}{2 \Lambda}\kappa^{\nu_{4}\nu_{i}}_{Z}\sigma_{\mu\nu}q^{\nu}P_L\nu_{4}Z^{\mu}+h.c.$
\end{itemize}
The effective Lagrangian for the magnetic type FCNC of the fourth generation quarks is

\begin{itemize}
\item ${\cal L}_{nc}=\left(\frac{\kappa^{q_4 q_{i}}_{\gamma}}{\Lambda}\right) e_{q}g_{e}\bar{q}_{4}\sigma_{\mu\nu}q_{i} F^{\mu\nu}+\left(\frac{\kappa^{q_4 q_{i}}_{Z}}{2\Lambda}\right) g_{Z}\bar{q}_{4}\sigma_{\mu\nu}q_{i} Z^{\mu\nu}+\left(\frac{\kappa^{q_4 q_{i}}_{g}}{\Lambda}\right) g_{s}\bar{q}_{4}\sigma_{\mu\nu}T^{a}q_{i} G^{\mu\nu}_{a}+h.c.$ 
\end{itemize}

In above equations, $\kappa_{W}$, $\kappa_{Z}$, $\kappa_{\gamma}$ and $\kappa_{g}$ are the anomalous couplings for the corresponding boson. $\Lambda$ is the cutoff scale for the new physics and  $P_L $ is the left handed projection operator; $g_{W}$ and $g_{Z}$ are the electroweak coupling constants. In the above equations
$\sigma_{\mu\nu} = i(\gamma_{\mu}\gamma_{\nu}-\gamma_{\nu}\gamma_{\mu})/2$. Obviously new interactions will lead to additional decay channels of the fourth family neutrino in addition to enhancement of some SM decay channels. In order to compute decay widths, branching ratios and cross sections, we have implemented the new interaction vertices into the CompHEP \cite{Boos:2004kh}. 

\subsubsection{Selected anomalous processes at $ep$ and $\gamma p$ colliders} 
 
\subsubsection{$ep\rightarrow l_4 X\rightarrow Z e (\gamma\mu)X$ processes at $ep$}
We consider $ep\rightarrow l_4 X \rightarrow \gamma\mu X$ and $ep\rightarrow l_4 X \rightarrow ZeX$ processes in this Section\,\cite{Ciftci:2006fw}. The latter process has SM backgrounds. Number of events for $m_{l_4}$ = 300 (700) GeV at $\sqrt{s}$ = 1.4 TeV and $\sqrt{s}$ = 3.74 TeV with 1 $fb^{-1}$ integrated luminosity are 240 (30) and 1170 (460), respectively.   However, in order to extract the fourth generation lepton signal and to suppress the background on the second process, we impose cuts on the eZ invariant mass. Thus, in calculations, we used $|m_{eZ}-m_{l_{4}}|<$25 
GeV for the mass range $m_{l_{4}}=100-1000$ GeV and $|m_{eZ}-m_{l_{4}}|<$50 GeV for the mass range of $1-2.6$ TeV with 
$p_{T}^{q}>$10 GeV cuts. All calculations for the signal and background were done by using the high-energy package CompHEP 
with CTEQ6L distribution function.

In order to examine the potential of the collider to search for the investigation of the anomalous interactions of the fourth SM 
family lepton in detail, we define statistical significance (SS) of the signal:
\vspace{ .1cm}
\begin{equation}
SS=\dfrac{\left | \sigma_{S+B}-\sigma_{B}\right |}{\sqrt\sigma_B}\sqrt L_{int}
\end{equation}\\[.1cm]where $L_{int}$ is the integrated luminosity of the collider. The values SS evaluated at each fourth SM family 
lepton mass points are shown in the last column of Table \ref{tab:bsm_ciftci_fourth.table1} and Table \ref{tab:bsm_ciftci_fourth.table2}. As seen from tables, one obtains good SS for the expected mass range of leptons. Also, we estimated achievable values of the coupling strengths by setting both minimum of $SS$ to three and minimum of signal events to five.


\begin{table}[h]
  \centering
  \begin{tabular}{|l|l|l|l|l|}
 
\hline
$m_{l_4}$(GeV) & $\sigma_{S+B}$(pb)& $\sigma_B$(pb)& SS & $(K/\Lambda)_{min}$ (TeV$^{-1}$) \\
\hline \hline
100 &0.13 &0.1 & 3& 1\\
200 & 0.49 & 0.09 & 42.16& 0.27 \\
300& 0.33 & 0.05 & 39.60& 0.28\\
400& 0.21 & 0.03 & 32.86& 0.30 \\
500& 0.13 & 0.015 & 15.49& 0.44\\
700& 0.039 & 0.009 & 10.00& 0.55\\
800& 0.019 & 0.005 & 6.26& 0.69\\
900& 0.0076 & 0.002 & 3.96& 0.87\\
1000& 0.0028 & 0.0011 & 1.62& -\\

\hline
\end{tabular}
\caption{ Total cross section of signal and background for $\sqrt{s}$ = 1.4 TeV and $(K/\Lambda)$ = 1TeV$^{-1}$ and achievable values of anomalous coupling strength.}
\label{tab:bsm_ciftci_fourth.table1}
\end{table}

\begin{table}[h]
  \centering
  \begin{tabular}{|l|l|l|l|l|}

\hline
$m_{l_4}$(GeV) & $\sigma_{S+B}$(pb) & $\sigma_B$(pb) & SS &$(K/\Lambda)_{min}$ (TeV$^{-1}$) \\
\hline \hline
200 & 1.234 &0.064 & 146.25& 0.15\\
400 & 0.856 & 0.026 & 162.77& 0.14 \\
600& 0.554 & 0.014 & 144.32& 0.15 \\
800& 0.339 & 0.009 & 110.00& 0.17 \\
1000& 0.32 & 0.03 & 52.94& 0.24 \\
1200& 0.19 & 0.02 & 38.01& 0.28\\
1400& 0.105 & 0.015 & 23.24& 0.36\\
1600& 0.062 & 0.012 & 14.43& 0.46\\
1800& 0.028 & 0.008 & 7.07& 0.65\\
2000& 0.016 & 0.006 & 4.08& 0.86\\
2200& 0.009 & 0.004 & 2.5& - \\
2400& 0.004 & 0.002 & 1.41& -\\
2600& 0.002 & 0.001 & 1& -\\
\hline
\end{tabular}
\caption{ Total cross section of signal and background for  $\sqrt{s}$ = 3.74 TeV, $(K/\Lambda)$ = 1TeV$^{-1}$ and achievable values of anomalous coupling strength.}
\label{tab:bsm_ciftci_fourth.table2}
\end{table}

LHeC will cover fourth family charged lepton up to 900 GeV while at Energy Frontier-ep collider the 
masses up to 2100 GeV can be reached. Hadron colliders including LHC are not very good place to investigate fourth family leptons \cite{1999fr} whereas, the capacity of lepton colliders are limited by their centre of mass energy.

\subsubsection{$ep\rightarrow \nu_4 X\rightarrow W (e,\mu) X$ processes at $ep$}

\begin{figure}[hb]
\includegraphics{bsm_ciftci_fourth_fig1}
\caption{\label{bsm_ciftci_fourth_fig1}Achievable values of anomalous coupling strength as a function of the fourth generation neutrino mass for $ep\rightarrow\nu_4X\rightarrow \mu W X$ process.}
\end{figure}

In this section, possible single productions of the fourth standard model generation neutrino via anomalous interactions at the future ep colliders are studied \cite{Ciftci:2007rv}.  In Ref. \cite{Ciftci:2007rv}, the Lagrangian for SM and the anomalous interactions of the fourth generation neutrino is presented; the experimental limits and the theoretical predictions on corresponding MNS matrix elements are discussed; the decay width and branching ratios of the fourth generation neutrino are evaluated. Production of the fourth generation neutrino at future ep colliders is studied: $ep\rightarrow\nu_4X\rightarrow \mu W X$ and $ep\rightarrow\nu_4X\rightarrow e W X$ processes as well as their SM backgrounds are considered; the statistical significance of the signal and achievable values of anomalous coupling strength are evaluated. 

New interactions, as implemented into the CompHEP, will lead to additional decay channels of the fourth family neutrino in addition to enhancement of some SM decay channels.  Experimental upper limit for $|V_{\nu_4l_i}|$ is 0.02 \cite{Kribs:2007nz}.  More realistic values for MNS matrix elements can be taken from Ref. \cite{Ciftci:2005gf}, namely: $V_{\nu_4\tau}$ = 2.34$\times10^{-5}$, $V_{{\nu_4}\mu}$ = 6.81$\times10^{-4}$, $V_{{\nu_4}e}$ = 4.64$\times10^{-4}$. Consequently, we have used these values at rest of our calculations.

Single anomalous production of the fourth SM generation neutrino is considered at ep colliders with $\sqrt{s}$ = 1.4 TeV (LHeC) and $\sqrt{s}$ = 3.74 TeV (Energy Frontier). We consider $ep\rightarrow\nu_4X\rightarrow \mu W X$ and $ep\rightarrow\nu_4X\rightarrow e W X$ processes as signatures of anomalous interactions of the fourth generation neutrino.  In order to extract the fourth generation neutrino signal and to suppress the background, we impose cuts on the eW invariant mass. Cuts of $|m_{eW}-m_{\nu_4}|<25$ GeV for the mass range $m_{\nu_4} =100-1000$ GeV and $|m_{eW}-m_{\nu_4}|<50$ GeV for the mass range of $1-2.6$ TeV together with $p_{T}^{q, l}>10$ GeV are applied. Since the process $ep\rightarrow\nu_4X\rightarrow \mu W X$ has no SM background one can use 10 events as a discovery limit (Fig. \ref{bsm_ciftci_fourth_fig1}). For the process $ep\rightarrow\nu_4X\rightarrow e W X$ we require $SS>5$ as a discovery criterion (Fig. \ref{bsm_ciftci_fourth_fig2}).
\begin{figure}[hb]
\includegraphics{bsm_ciftci_fourth_fig2}
\caption{\label{bsm_ciftci_fourth_fig2}Achievable values of anomalous coupling strength as a function of the fourth generation neutrino mass for $ep\rightarrow\nu_4X\rightarrow e W X$ process.}
\end{figure}

\subsubsection{$q_4\rightarrow \gamma q$ and $q_4\rightarrow Z q$ processes at $ep$ and $\gamma p$ colliders}

In this study, $e p \rightarrow e u_4 (d_4) X \rightarrow e q \gamma X$, $e p \rightarrow e u_4 (d_4) X \rightarrow q Z X \rightarrow e q \ell^+ \ell^- X$, $\gamma p \rightarrow u_4 (d_4) X \rightarrow q \gamma X$ and $\gamma p \rightarrow u_4 (d_4) X \rightarrow q Z X \rightarrow q \ell^+ \ell^- X$ processes (and their h.c.) are considered as  signatures of anomalous interactions of the fourth generation up and down type quarks ($q=u,c$ for $u_4$ and $q=d,s,b$ for $d_4$ and $\ell=e,\mu$) \cite{Ciftci:2009it}. We choose the following cut selection criteria for the first and third processes:  $P_T\:>\:10$ GeV for the electron, $P_T\:>\:80$ GeV for photon, $P_T\:>\:20$ GeV for the jet, $\left|\eta_{j,e,\gamma}\right|\:<\:2.5$, $\Delta R_{j,\ell,\gamma}\:>\:0.4$ between the electron, photon and jet. Similar but slightly different cuts are applied for the second and fourth processes: $P_T\:>\:50$ GeV for leptons, $P_T\:>\:20$ GeV for the jet, $\left|\eta_{j,\ell,\gamma}\right|\:<\:2.5$, $\Delta R_{j,\ell}\:>\:0.4$ between the lepton and jet.

For our purposes, the electron beam energy is chosen as 60 GeV. For the choice of a cw mode superconducting energy recovery e-linac with an upgraded LHC, the integrated luminosity for a year has been estimated $10  fb^{-1}$. However, for the choice of pulsed superconducting e-linac with an upgraded LHC, the integrated luminosity per year has been determined as $4.1 fb^{-1}$. While the first choice has a better luminosity, it is not possible to found a gamma-p collider on base of it. The real gamma production through the Compton backscattering technique on the base of the ep collider is possible on the second choice. In this case, the integrated luminosity of $\gamma p$ collider reaches the maximum value of $2.665 fb^{-1}$. 

One can compute achievable values of the coupling strengths by setting both minimum of $SS$ to three and minimum of signal events to five. The results are presented at Figure \ref{bsm_ciftci_fourth_fig3} for various fourth generation quark masses. The solid line at figure 4a corresponds to $\kappa_\gamma/\Lambda$ values independent of $\kappa_Z/\Lambda$. The rest of lines are for $\kappa/\Lambda=\kappa_\gamma/\Lambda=\kappa_Z/\Lambda$. When anomalous coupling strengths for electromagnetic and weak interactions are not equal, one can obtain them by using  $\gamma p \rightarrow u_4 (d_4) X \rightarrow q Z X \rightarrow q \ell^+ \ell^- X$ process (Fig. \ref{bsm_ciftci_fourth_fig3}c).

\begin{figure}[hb]
\vspace{-0.2cm}
{\includegraphics[width=7cm]{bsm_ciftci_fourth_fig3a}} \ \ \ \ \ \ \ \ \ \
{\includegraphics[width=7cm]{bsm_ciftci_fourth_fig3b}} \ \ \ \ \ \ \ \ \ \  
{\includegraphics[width=7cm]{bsm_ciftci_fourth_fig3c}} 
\vspace{-0.2cm}
\caption{The achievable values of the anomalous coupling strength at $ep$ and $\gamma p$ colliders for a) $q_4 \rightarrow \gamma q$ anomalous process and (b) $q_4 \rightarrow Z q$ anomalous process as a function of the $q_{4}$ mass; (c) the reachable values of anomalous photon and Z couplings with $L_{int}=4.1$ fb$^{-1}$. \protect\label{bsm_ciftci_fourth_fig3}}
\end{figure}


\subsubsection{Conclusion}

Combining results of studies on anomalous single production of the fourth SM generation charged lepton and neutrino  at future ep colliders we conclude that they have promising potential on the subject. For example, if $m_{\nu_4}= m_{l_4}= 500$ GeV and $(\kappa/\Lambda)$ = 1TeV$^{-1}$, the numbers of produced events are 740 for $ep\rightarrow\nu_4X\rightarrow e W X$ and 1100 for $ep\rightarrow l_4X\rightarrow e Z X$ at $\sqrt{s} = 1.4$ TeV with $L_{int}=10$ fb$^{-1}$. Finally, LHeC cover $m_{\nu_4, l_4}< 1$ TeV, whereas Energy Frontier enlarge the region up to 2 TeV.

When the anomalous coupling  for strong interactions is close to one, $ep$ and $\gamma p$ colliders are almost blind to anomalous interactions of the fourth generation quarks. In this case, hadron colliders like LHC will be discovery machines. $ep$ and $\gamma p$ colliders enable us to investigate effects of both anomalous couplings of electromagnetic and weak interactions for $\kappa^{q_{i}}_{g}=0$. This type anomalous interactions takes place through Weizsacker-Williams photons or Z boson at the LHC. However, LHC based $ep$ and $\gamma p$ colliders have better observation reaches of anomalous couplings compare to the LHC.

The advantage of the $\gamma p$ collider with respect to $ep$ collider for single production of $q_4$ is obvious even with $1/100$ (for $q_4\rightarrow \gamma q$) and $1/10$ (for $q_4\rightarrow Z q$) of luminosity of ep collider.

$ep$ and  $\gamma p$ colliders are almost  only place to investigate  anomalous coupling strengths of electroweak interactions separately.
  Such as $\kappa_{Z}^{q q_4}$, $\kappa_{\gamma}^{q q_4}$, $\kappa_{Z}^{l l_4}$, $\kappa_{\gamma}^{l l_4}$ and $\kappa_{W}^{l \nu_4}$ 

\clearpage

==> physics/bsm_ciftci_qstar.tex <==
\newpage
\subsection{Production of excited quark at $\gamma p$ collider based on the Large Hadron
  electron Collider}

\vspace{0.2cm}
\noindent
Rena Çiftçi ~~~~~~~~~~~~~~~~~~ Ankara U. 10.08.2010
%------------------------------------
%
% Start of the text proper
%

Composite models are foreseen to explain repeated generations of quarks and leptons. Excited quarks with rich spin and weak isospin spectra are unavoidable outcome of preonic models \cite{Terazawa:1981eg,Renard:1982ya,DeRujula:1983ak,Kuhn:1984rj,Baur:1987ga,Baur:1989kv}. Therefore, observation of excited quarks and investigation of their properties will give opportunity to determine mechanism of compositeness of quarks and leptons. 

D0 experiment at Fermilab Tevatron collider excludes excited quarks with mass region below 775 GeV for two jet decays at $p \bar{p}$ collisions with the assumption of $f=f'=f_s=\Lambda/m^*$ \cite{Abazov:2003tj}. Also, mass region below 760 GeV are excluded for $jj$ decay by CDF experiment \cite{Abe:1995jz,Abe:1997hm}. Recently, D0 experiment has assumed $q^*$ production via $q g$ fusion and via contact interactions and looked at Z jet decay to obtain exclusion of below 510 GeV \cite{Abazov:2006nr}. The quoted limit is for $\Lambda = m^*$.
 
The best place to discover the excited quark is hadron colliders like CERN Large Hadron Collider (LHC) \cite{Baur:1989kv,Cakir:1999nu}. Very high mass reach and low coupling values are possible at LHC. Unfortunately, LHC does not permit accurate investigation of the properties of the excited quarks. Excited quarks can be pairly produced at $e^+e^-$ colliders. However, their production is restricted by relatively low center of mass energy of lepton colliders. At this point of view $ep$ and $\gamma p$ colliders are more advantageous because the excited quark is single produced at them. In addition to clearer signal environment, it is possible to investigate properties of the excited quarks with photo-production \cite{Bagger:1984su,Cashmore:1985xn,Jikia:1989gj}. In $ep$ colliders, Weisz\"{a}cker-Williams photons are used to produce excited quarks. However, their spectrum is concentrated at lower energies. Fortunately, it is possible to produce real photons by colliding laser photons with high energy electrons. Resulting Compton backscattered photons are produced with high polarization and a spectrum with most of photons carrying about 80 percent of electron energy \cite{cGinzburg:1981vm,Ginzburg:1982yr,Telnov:1989sd}. Recently, LHC based linac-ring type $ep$ colliders were proposed in refs. \cite{Arik:2003wy,Sultansoy:2003wv,Schulte:2004qw} with the names of QCD Explorer with $\sqrt{s}=1.4$ TeV and Energy Frontier $ep$ collider with $\sqrt{s}=3.74$ TeV. Their luminosities are determined as $1$ fb$^{-1}$ and $10$ fb$^{-1}$ depending on choosen accelerator configurations for LHeC \cite{ciftci2.21}, as well as $100$ pb$^{-1}$ and $1$ fb$^{-1}$ for Energy Frontier \cite{ciftci2.19}. In Refs. \cite{ciftci2.22,Aksakal:2006fa,Ciftci:2007zza,ciftci2.25}, the feasibility of $\gamma p$ colliders based on LHeC and Energy Frontier $ep$ colliders is shown. The maximum possible luminosity of the $\gamma p$ colliders is limited by maximum possible yield of high energy photon production per electron, which is $0.6$. Therefore, the integrated luminosity per year of $\gamma p$ collider based on LHeC (Energy Frontier) may be obviously taken as $0.6$ fb$^{-1}$ and $6$ fb$^{-1}$ ($60$ pb$^{-1}$ and $0.6$ fb$^{-1}$).

$\gamma p \rightarrow q^{*} X \rightarrow g q X$ and $\gamma p \rightarrow q^{*} X \rightarrow \gamma q X$ processes as well as their SM backgrounds are considered; the statistical significance of the signal and achievable values of compositeness parameters $f_s$, $f$ and $f^\prime $ are evaluated.
 %
\subsubsection{Excited quark involved interactions}
%
Excited quarks will have vertices with SM quark and gauge bosons (photon, gluon, Z or W bosons). They can be produced at $ep$ and $\gamma p$ colliders via quark photon fusion. Interactions involved excited quark can be described as below \cite{Baur:1989kv}:
\begin{equation}
L=\frac{1}{2\Lambda}\bar{q}^*_R \sigma^{\mu\nu}\left(g_s f_s\frac{\lambda^a}{2}G^a_{\mu\nu}+g f \frac{\tau}{2}\cdot W_{\mu\nu}+g'f'\frac{Y}{2} B_{\mu\nu}\right)q_L+h.c.
\end{equation}
where $G^a_{\mu\nu}$, $W_{\mu\nu}$ and $B_{\mu\nu}$ are the field-strength tensors of the gluon, the SU(2) and the U(1) gauge fields; $\lambda^a$, $\tau$ and $Y$ are the corresponding gauge structure constants; $g_s$, $g=e/{sin\theta_W}$ ($e=\sqrt{4 \pi \alpha}$) and $g'=e/{cos\theta_W}$ are the strong and electroweak gauge couplings; $f_s$, $f$ and $f'$ are parameters determined by the composite dynamics.

In order to perform computations for the excited quarks, above Lagrangian given in the above equation has been implemented into the CompHEP \cite{Boos:2004kh}.  In the calculations, $\Lambda=m^{*}$ and $f=f'=f_s=1$ have been taken. More than 80 percent of excited quarks decay into quark and gluon.

\subsubsection{The excited quark production at $\gamma p$ colliders}
%
In this study only $\gamma q \rightarrow q^{*} \rightarrow g q$ and $\gamma q \rightarrow q^{*} \rightarrow \gamma q$ processes are considered as signatures (at parton level) of the excited quarks at $\gamma p$ colliders. These signatures will be observed as dijet and photon-jet at the detector, respectively.
For both the dijet and photon-jet processes, the pseudorapidity of jets is taken $\left| \eta_j \right|<2.5$; the pseudorapidity of photon is taken $\left| \eta_{\gamma} \right|<2.5$; separation between jets is taken $\Delta R_{j j}>0.7$ and separation between photon and jet is taken $\Delta R_{j \gamma}>0.4$ as detector limitations. One should note that with above detector cuts the SM background cross section originate from the processes: $\gamma q\rightarrow g q$ (where $q=u,d,c,s$) contributes \%8, $\gamma \bar{q}\rightarrow g \bar{q}$ (where $q=u,d,c,s$) contributes \%8, and $\gamma g\rightarrow q \bar{q}$ (where $q=u,d,c,s,t,b$) contributes \%84 in $\gamma p\rightarrow j j X$ process; $\gamma q\rightarrow \gamma q$ (where $q=u,d,c,s$) contributes \%51, and $\gamma \bar{q}\rightarrow \gamma \bar{q}$ (where $q=u,d,c,s$) contibutes \%49 in $\gamma p\rightarrow \gamma j X$ process. In order to extract the excited quark signal and to suppress the SM background, we impose transverse momentum cut to jets also. Various $p_T$ cuts are applied to both signal and background processes. The most of the SM backgrounds reduced with $p_T$ cut; optimal cut value for transverse momentum seems to be about one third of the excited quark mass. Consequently, in the numerical calculations transverse momenta of jets are taken bigger than $m^*/3$ to suppress the background. One should not that, transverse momentum cut is more efficient for LHeC. For example, while the dijet SM background is decreased by order of $10^5$ for Energy Frontier, it is reduced with more than $10^7$ factor for LHeC. By applying above detector and $p_T$ cuts the computed signal and background cross sections for the $\gamma p \rightarrow q^{*} X \rightarrow jj X$ process are given in Tables \ref{tab:ciftci2.table1} and \ref{tab:ciftci2.table2} for $\sqrt{s_{max}}$ = 1.27 TeV and $\sqrt{s_{max}}$ = 3.41 TeV options, respectively. Similar calculations for the $\gamma p \rightarrow q^{*} X \rightarrow \gamma j X$ process are presented in Tables \ref{tab:ciftci2.table3} and \ref{tab:ciftci2.table4}. In the last two columns of these tables, the statistical significance (SS) values of the excited quark signal (evaluated from $SS=(\sigma_{S}/\sqrt{\sigma_B})\sqrt{L_{int}}$, where $L_{int}$ is the integrated luminosity of the collider) are given.  

\begin{table}

\begin{tabular}{|c|cc|cc|}
\hline
$m^{*}$ & \multicolumn{2}{c|} {$\gamma p \rightarrow u^{*} X \rightarrow jj X$($\gamma p \rightarrow d^{*} X \rightarrow jj X$)} & \multicolumn{2}{c|} {$SS$} \\
\cline{2-3}\cline{4-5}
(GeV) & $\sigma_{S}$ (pb) & $\sigma_{B}$ (pb) & $\textsl{L}_{int}=0.6$ fb$^{-1}$ & $\textsl{L}_{int}=6$ fb$^{-1}$ \\ 
\hline \hline

600 &  6.310  (0.700) & 2.58 &  96.23 (10.67) &  304.30 (33.76) \\
700 &  2.350  (0.210) & 1.08 &  55.39 (4.95) &  175.16 (15.65) \\
800 &  0.750  (0.056) & 0.45 &  27.39 (2.04) &  86.60 (6.47) \\
900 &  0.201  (0.011) & 0.20 &  11.01 (0.60) &  34.81 (1.91) \\
1000 & 0.040  (0.002) & 0.082 &  3.42 (0.17) &  10.82 (0.54) \\
1100 & 0.0050  (0.0002) & 0.032 &  0.68 (0.03) &  2.17 (0.09) \\ \hline
\end{tabular}
\caption{The signal and background cross sections of the excited quark $jj$ channel and corresponding SS for LHeC based $\gamma p$ collider.}
\label{tab:ciftci2.table1}
\end{table}

\begin{table}
\begin{tabular}{|c|cc|cc|}
\hline
$m^{*}$ & \multicolumn{2}{c|} {$\gamma p \rightarrow u^{*} X \rightarrow jj X$($\gamma p \rightarrow d^{*} X \rightarrow jj X$)} & \multicolumn{2}{c|} {$SS$} \\
\cline{2-3}\cline{4-5}
(GeV) & $\sigma_{S}$ (pb) & $\sigma_{B}$ (pb) & $\textsl{L}_{int}=60$ pb$^{-1}$ & $\textsl{L}_{int}=600$ pb$^{-1}$ \\ 
\hline \hline

600 &  33.60  (6.34) & 33.73 &  44.8 (8.5) &  141.7 (26.7) \\
800 &  14.28  (2.46) & 10.27 &  34.5 (5.9) &  109.1 (18.8) \\
1000 &  7.16  (1.08) & 3.90 &  28.1 (4.2) &  88.8 (13.4) \\
1200 &  3.81  (0.51) & 1.68 &  22.8 (3.0) &  72.0 (9.6) \\
1400 &  2.07  (0.25) & 0.78 &  18.2 (2.2) &  57.4 (6.9) \\
1600 &  1.12  (0.12) & 0.39 &  13.9 (1.5) &  43.9 (4.7) \\
1800 & 0.59  (0.053) & 0.20 &  10.2 (0.92) &  32.3 (2.9) \\
2000 & 0.29  (0.022) & 0.10 &  7.1 (0.54) &  22.5 (1.7) \\
2200 & 0.13  (0.0085) & 0.057 &  4.2 (0.28) &  13.3 (0.87) \\
2400 & 0.052  (0.0027) & 0.030 &  2.3 (0.12) &  7.4 (0.38) \\
2600 & 0.018  (0.00072) & 0.016 &  1.1 (0.044) &  3.5 (0.14) \\ \hline
\end{tabular}
\caption{The signal and background cross sections of the excited quark $jj$ channel and corresponding SS for Energy Frontier $ep$ based $\gamma p$ collider.}
\label{tab:ciftci2.table2}
\end{table}

\begin{table}
\begin{tabular}{|c|cc|cc|}
\hline
$m^{*}$ & \multicolumn{2}{c|} {$\gamma p \rightarrow u^{*} X \rightarrow \gamma j X$($\gamma p \rightarrow d^{*} X \rightarrow \gamma j X$)} & \multicolumn{2}{c|} {$SS$} \\
\cline{2-3}\cline{4-5}
(GeV) & $\sigma_{S}$ (pb) & $\sigma_{B}$ (pb) & $\textsl{L}_{int}=0.6$ fb$^{-1}$ & $\textsl{L}_{int}=6$ fb$^{-1}$ \\ 
\hline \hline

600 &  0.17  (0.0045) & 0.045 &  19.6 (0.52) &  62.1 (1.6) \\
700 &  0.062  (0.0014) & 0.022 &  10.2 (0.23) &  32.4 (0.73) \\
800 &  0.020  (0.00037) & 0.0099 &  4.9 (0.091) &  15.6 (0.29) \\
900 &  0.0054  (0.000078) & 0.0045 &  2.0 (0.028) &  6.2 (0.090) \\
1000 & 0.0011  (0.000011) & 0.0020 &  0.60 (0.0060) &  1.9 (0.019) \\ \hline
\end{tabular}
\caption{The signal and background cross sections of the excited quark $\gamma j$ channel and corresponding SS for LHeC based $\gamma p$ collider.}
\label{tab:ciftci2.table3}
\end{table}

\begin{table}
\begin{tabular}{|c|cc|cc|}
\hline
$m^{*}$ & \multicolumn{2}{c|} {$\gamma p \rightarrow u^{*} X \rightarrow \gamma j X$($\gamma p \rightarrow d^{*} X \rightarrow \gamma j X$)} & \multicolumn{2}{c|} {$SS$} \\
\cline{2-3}\cline{4-5}
(GeV) & $\sigma_{S}$ (pb) & $\sigma_{B}$ (pb) & $\textsl{L}_{int}=60$ pb$^{-1}$ & $\textsl{L}_{int}=600$ pb$^{-1}$ \\ 
\hline \hline

600 &  0.78  (0.041) & 0.28 &  11.4 (0.60) &  36.1 (1.9) \\
800 &  0.38  (0.016) & 0.11 &  8.9 (0.37) &  28.1 (1.2) \\
1000 &  0.19  (0.0075) & 0.051 &  6.5 (0.26) &  20.6 (0.81) \\
1200 &  0.10  (0.0036) & 0.026 &  4.8 (0.17) &  15.2 (0.55) \\
1400 &  0.060  (0.0017) & 0.014 &  3.9 (0.11) &  12.4 (0.35) \\
1600 &  0.033  (0.00085) & 0.0078 &  2.9 (0.075) &  9.2 (0.24) \\
1800 & 0.017  (0.00039) & 0.0044 &  2.0 (0.046) &  6.3 (0.14) \\
2000 & 0.0086  (0.00017) & 0.0024 &  1.4 (0.027) &  4.3 (0.085) \\
2200 & 0.0039  (0.000064) & 0.0014 &  0.81 (0.013) &  2.6 (0.042) \\ \hline

\end{tabular}

\caption{The signal and background cross sections of the excited quark $\gamma j$ channel and corresponding SS for Energy Frontier $ep$ based $\gamma p$ collider.}
\label{tab:ciftci2.table4}
\end{table}
         
\begin{figure}
{\includegraphics[width=8.15cm]{bsm_ciftci_qstar_fig1a}}
{\includegraphics[width=8.15cm]{bsm_ciftci_qstar_fig1b}}
\caption{Observation reach at $3\sigma$ for coupling and excited quark mass ($jj$ channel) at $\gamma p$ collider with (a) $\sqrt{s}$ = 1.27 TeV and (b) $\sqrt{s}$ = 3.41 TeV. \protect\label{bsm_ciftci_1star_fig1}}
\end{figure} 

\begin{figure}
{\includegraphics[width=8.15cm]{bsm_ciftci_qstar_fig2a}}
{\includegraphics[width=8.15cm]{bsm_ciftci_qstar_fig2b}}
\caption{Observation reach at $3\sigma$ for coupling and excited quark mass ($\gamma j$ channel) at $\gamma p$ collider with (a) $\sqrt{s}$ = 1.27 TeV and (b) $\sqrt{s}$ = 3.41 TeV. \protect\label{bsm_ciftci_1star_fig2}}
\end{figure}

Achievable mass and coupling values for the excited quark are established by requiring $SS\geq3$ as an observation criterion. For the process $\gamma p \rightarrow q^{*} X \rightarrow jj X$ it is seen from Tables \ref{tab:ciftci2.table1} and \ref{tab:ciftci2.table2}, that LHeC will cover masses of $u^{*}$ excited quark up to 1000 GeV (1080 GeV) with ${L}_{int}=0.6$ fb$^{-1}$ (6 fb$^{-1}$) for $\Lambda=m^{*}$ and $f=f'=f_s=1$, whereas Energy Frontier $\gamma p$ collider will extend the mass region up to $m_{u^{*}}=2320$ GeV (2620 GeV) with ${L}_{int}=60$ pb$^{-1}$ (600 pb$^{-1}$). Similarly, LHeC will reach $m_{d^{*}}=755$ GeV (870 GeV) with ${L}_{int}=0.6$ fb$^{-1}$ (6 fb$^{-1}$). Corresponding limit for Energy Frontier is 1200 GeV (1790 GeV) with ${L}_{int}=60$ pb$^{-1}$ (600 pb$^{-1}$). Observation reach of compositeness parameters $f_s$, $f$ and $f^\prime $ as a function of the excited quark mass for process under consideration is presented in Fig. \ref{bsm_ciftci_1star_fig1} for different $\gamma p$ colliders. As seen from the figure, it will be possible to probe compositeness parameters down to 0.1 depending on the mass.  

For the process $\gamma p \rightarrow q^{*} X \rightarrow \gamma j X$ Tables \ref{tab:ciftci2.table3} and \ref{tab:ciftci2.table4} show that, excited up quark will be observed up to $m_{u^{*}}=855$ GeV (965 GeV) at QCD Explorer with ${L}_{int}=0.6$ fb$^{-1}$ (6 fb$^{-1}$), whereas these limits becomes 1570 GeV (2140 GeV) for Energy Frontier with ${L}_{int}=60$ pb$^{-1}$ (600 pb$^{-1}$). Figure \ref{bsm_ciftci_1star_fig2} shows observation reach of compositeness parameters $f_s$, $f$ and $f^\prime $ as a function of the excited up quark mass. Observation of $d^{*}$ excited quark is not possible at this channel with given collider parameters (see Tables \ref{tab:ciftci2.table3} and \ref{tab:ciftci2.table4}).         



\subsubsection{Conclusion}

$\gamma p$ colliders are complementary to hadron colliders like LHC. While LHC is the best place for discovery of excited quarks in a very wide range of masses, $\gamma p$ colliders such as ones that based on LHeC and Energy Frontier $ep$ collider are essential for detailed studies of properties of the excited quark interactions. Concerning the criterion $SS\geq3$ and taking $\Lambda=m^{*}$ and $f=f'=f_s=1$, the excited quark can be observed up to 2.6 TeV at future $\gamma p$ colliders. In this paper, only $\gamma p \rightarrow q^{*} X \rightarrow jj X$ and $\gamma p \rightarrow q^{*} X \rightarrow \gamma j X$ channels are considered as signatures. It is determined that the former channel is more promising for both $u^{*}$ and $d^{*}$ than latter one. For example, if $m_{q^{*}}=850$ GeV, the numbers of produced jet jet (photon jet) events are 2424 (66) for $u^{*}$ and 162 (not observable) for $d^{*}$ at $\sqrt{s_{max}}$ = 1.27 TeV with ${L}_{int}=6$ fb$^{-1}$. If $m_{q^{*}}=1700$ GeV, the numbers of produced jet jet (photon jet) events are 486 (14) for $u^{*}$ and 47 (not observable) for $d^{*}$ at $\sqrt{s_{max}}$ = 3.41 TeV with ${L}_{int}=600$ pb$^{-1}$. 

Also, investigation of pseudorapidity shows that LHeC based $\gamma p$ collider requires a forward detector designed for it. Meanwhile one can use a detector similar to ATLAS for Energy Frontier $\gamma p$ collider.        


\clearpage

==> physics/bsm_ocakir_anotop.tex <==
\newpage
\subsection{Anomalous single top production at the LHeC based $\gamma$p collider}

\vspace{0.2cm}
\noindent
% I.T. Cakir (Ankara Univ.), O. Cakir (Ankara Univ.), S. Sultansoy (TOBB ETU) ~~~~~~~~~~~~~~~~~~17.08.2010

%------------------------------------
%
% Start of the text proper
%
The top quark is considered to be the most sensitive to the new physics
beyond the Standard Model (BSM) because it is the heaviest available
particle of the Standard Model (SM). If the BSM is associated with
the mass generation, the top quark interactions will be sensitive
to the mechanism of dynamical symmetry breaking. The precise measurement
of the couplings between SM bosons and fermions provides powerful
tool for the search of the BSM physics. The effects of new physics
on the top quark couplings are expected to be larger than that on
any other fermions, and deviations with respect to the SM predictions
might be detectable~\cite{AguilarSaavedra:2008zc}. A possible anomalous $tqV$ ($V=g,\gamma,Z$
and $q=u,c$) couplings can be generated through a dynamical mass
generation ~\cite{Fritzsch:1999rd}. They have a similar chiral structure as the
mass terms, and the presence of these couplings would be interpreted
as signals of new interactions. This motivates the study of top quarks'
flavour changing neutral current (FCNC) couplings at present and future
colliders.

Current experimental constraints at 95\% C.L. on the anomalous top
quark couplings are ~\cite{Amsler:2008zzb}: $BR(t\rightarrow\gamma u)<0.0132$
and $BR(t\rightarrow\gamma u)<0.0059$ from HERA; $BR(t\rightarrow\gamma q)<0.041$
from LEP and $BR(t\rightarrow\gamma q)<0.032$ from CDF. The HERA
has much higher sensitivity to $u\gamma t$ than $c\gamma t$ due
to more favorable parton density: the best limit is obtained from
the ZEUS experiment.

The top quarks will be produced in large numbers at the Large Hadron
Collider (LHC), therefore the couplings of the top quark can be probed
with a great precision. For a luminosity of 1 fb$^{-1}$ (100 fb$^{-1}$)
the expected ATLAS sensitivity to the top quark FCNC decay is $BR(t\to q\gamma)\sim10^{-3}(10^{-4})$
~\cite{Aad:2009wy,:1999fr}. The production of top quarks by FCNC interactions at
hadron colliders has been studied in~\cite{Han:1996ce,Malkawi:1995dm,Tait:1996dv,Han:1998tp,
Tait:2000sh,Liu:2004bb,Liu:2005dp,Cao:2007bx,Cao:2007dk,Ferreira:2008cj,Yang:2008sb,
Han:2009zm,Cao:2008vk}, $e^{+}e^{-}$colliders
in~\cite{Fritzsch:1999rd,Obraztsov:1997if,Han:1998yr,Cao:2002si,AguilarSaavedra:2004wm} 
and lepton-hadron collider in ~\cite{Fritzsch:1999rd,Alan:2002wv,Ashimova:2006zc,Aaron:2009vv}. LHC will
give an opportunity to probe $BR(t\rightarrow ug)$ down to $5\times10^{-3}$
~\cite{Cakir:2005rf}; ILC/CLIC has the potential to probe $BR(t\rightarrow q\gamma)$
down to $10^{-5}$ ~\cite{MoortgatPick:2005cw}.

The linac-ring type colliders present the sole realistic way to TeV
scale in lepton-hadron collisions ~\cite{Sultansoy:2003wv} and advantage to construct
$\gamma p$ colliders on their basis ~\cite{Sultanov:1989zx,Alekhin:1988iu,Ciftci:1995ea,Ciftci:2000xg,Aksakal:2006fa}. Recently this opportunity
is widely discussed in the framework of the LHeC project ~\cite{Dainton:2006wd}.
Two stages of the LHeC are considered: QCD Explorer ($E_{e}=50-100$
GeV) and Energy Frontier ($E_{e}>250$ GeV). First stage is mandatory
for two reasons: to provide precision PDF's for adequate interpretation
of LHC data and to enlighten fundamentals of QCD.

The potential of LHeC based $\gamma p$ collider to search for anomalous
top quark interactions has been investigated~\cite{Cakir:2009rq}. The effective
Lagrangian involving anomalous $t\gamma q$ $(q=u,c)$ interactions
is given by ~\cite{Cakir:2005rf}.

\begin{equation}
L=-g_{e}\sum_{q=u,c}{\displaystyle Q_{q}\frac{\kappa_{q}}{\Lambda}\bar{t}\sigma^{\mu\nu}(f_{q}+h_{q}\gamma_{5})qA_{\mu\nu}+h.c.}\label{eq:1}\end{equation}
 where $A_{\mu\nu}$ is the usual photon field tensor, $\sigma_{\mu\nu}=\frac{i}{2}(\gamma_{\mu}\gamma_{\nu}-\gamma_{\nu}\gamma_{\mu})$,
$Q_{q}$ is the quark charge, in general $f_{q}$ and $h_{q}$ are
complex numbers, $g_{e}$ is electromagnetic coupling constant, $\kappa_{q}$
is real and positive anomalous FCNC coupling and $\Lambda$ is the
new physics scale. The neutral current magnitudes in the Lagrangian
satisfy $|(f_{q})^{2}+(h_{q})^{2}|=1$ for each term. The anomalous
decay width can be calculated as

\begin{equation}
\Gamma(t\rightarrow q\gamma)=(\frac{\kappa_{q}}{\Lambda})^{2}\frac{2}{9}\alpha_{em}m_{t}^{3}\label{eq:2}\end{equation}


Taking $m_{t}=173$ GeV and $\alpha_{em}=0.0079$, the anomalous decay
width $\approx9$ MeV for $\kappa_{q}/\Lambda=1$ TeV$^{-1}$is calculated,
while the SM decay width is about 1.5 GeV. For numerical calculations
anomalous interaction vertices are implemented into the CalcHEP package
~\cite{Pukhov:2004ca} with the CTEQ6M ~\cite{Pumplin:2002vw}. The Feynman diagrams for the
subprocess $\gamma q\rightarrow W^{+}b$, where $q=u,c$ are shown
in Fig. \ref{fig:1}. First three diagrams correspond to irreducible
background and the last one to signal.

The main background comes from associated production of $W$ boson
and the light jets. Here, b-tagging efficiency is used as 60\% and
the mistagging factors for light ($u,d,s$) and $c$ quarks are taken
as 0.01 and 0.1, respectively.

The differential cross sections for the final state jets are given
in Fig. \ref{fig:2} ($\kappa/\Lambda=0.04$ TeV$^{-1}$) for $E_{e}=70$
GeV and $E_{p}=7000$ GeV assuming $\kappa_{u}=\kappa_{c}=\kappa$.
It is seen that the transverse momentum distribution of the signal
has a peak around 70 GeV in Fig. \ref{fig:2} .

%
\begin{figure}[hb]
\centering{\includegraphics[clip=,width=0.35\textwidth]{ocakir_anomtop_fig1}\caption{Feynman diagrams for $\gamma q\rightarrow W^{+}b$, where $q=u,c$.\label{fig:1}}}

\end{figure}


%
\begin{figure}[hb]
\centering{\includegraphics[clip=,width=0.35\textwidth,scale=0.6]{ocakir_anomtop_fig2}\caption{The transverse momentum distribution of the final state jet for the
signal and background processes. The differential cross section includes
the b-tagging efficiency and the rejection factors for the light jets.
The center of mass energy $\sqrt{s_{ep}}=1.4$ TeV and $\kappa/\Lambda=$0.04
TeV $^{-1}$\label{fig:2}. }}

\end{figure}


The $p_{T}$ cut slightly reduce the signal $(\sim30\%$ for $p_{T}>50$
GeV), whereas the background is essentially reduced (factor 4-6) .
In order to improve the signal to background ratio further one can
use invariant mass ($W+jet$) cut around top mass. In Table \ref{anotop_tab:1},
the cross sections for signal and background processes are given using
both $p_{T}$ and invariant mass cuts $(M_{Wb}=150-200$ GeV).

%
\begin{table}[ht]
\caption{The cross sections (in pb) according to the $p_{T}$ cut and invariant
mass interval $(M_{Wb}=150-200$ GeV) for the signal and background
at $\gamma p$ collider based on the LHeC with $E_{e}=70$ GeV and
$E_{p}=$7000 GeV. \label{anotop_tab:1}}


\begin{tabular}{|c|c|c|c|}
\hline
$\kappa/\Lambda=0.01$ TeV$^{-1}$  & $p_{T}>20$ GeV  & $p_{T}>40$ GeV  & $p_{T}>50$ GeV\tabularnewline
\hline
\hline
Signal  & $8.86\times10^{-3}$  & $7.54\times10^{-3}$  & $6.39\times10^{-3}$\tabularnewline
\hline
Background: $W^{+}b$  & $1.73\times10^{-3}$  & $1.12\times10^{-3}$  & $7.69\times10^{-4}$\tabularnewline
\hline
Background: $W^{+}c$  & $3.48\times10^{-1}$  & $2.30\times10^{-1}$  & $1.63\times10^{-1}$\tabularnewline
\hline
Background: $W^{+}jet$  & $1.39\times10^{-1}$  & $9.11\times10^{-2}$  & $6.38\times10^{-2}$\tabularnewline
\hline
\end{tabular}
\end{table}


In order to calculate the statistical significance (\emph{SS}) we
use following formula ~\cite{Ball:2007zza} :

\begin{equation}
SS=\sqrt{2\left[(S+B)\ln(1+\frac{S}{B})-S\right]}\label{eq:3}\end{equation}
 where $S$ and $B$ are the numbers of signal and background events,
respectively. Results are presented in Table \ref{anotop_tab:2} for different
$\kappa/\Lambda$ and luminosity values. It is seen that even with
$2$ fb$^{-1}$ the LHeC based $\gamma p$ collider will provide $5\sigma$
discovery for $\kappa/\Lambda=0.02$ TeV$^{-1}$.

%
\begin{table}[ht]
\caption{The signal significance ($SS$) for different values of $\kappa/\Lambda$
and integral luminosity for $E_{e}=70$ GeV and $E_{p}=$7000 GeV
(the numbers in parenthesis correspond to $E_{e}=140$ GeV). \label{anotop_tab:2}}

\begin{tabular}{|c|l|c|}
\hline
$SS$  & $L=2$ fb$^{-1}$  & $L=10$ fb$^{-1}$\tabularnewline
\hline
\multicolumn{1}{||c||}{$\kappa/\Lambda=0.01$ TeV$^{-1}$} & 2.58 (2.88)  & 5.79 (6.47)\tabularnewline
\hline
$\kappa/\Lambda=0.02$ TeV$^{-1}$  & 5.26 (5.92)  & 11.78 (13.25)\tabularnewline
\hline
\end{tabular}
\end{table}

Up to now, we assume $\kappa_{u}=\kappa_{c}=\kappa$. However, it
is a matter of interest to analyze the $\kappa_{u}\neq\kappa_{c}$
case. Being different from HERA where anomalous single top production
is dominated by valence $u$-quarks, at LHeC energy region $c$-quark
contribution becomes comparable with the $u$-quark contribution.
Therefore, the sensitivity to $\kappa_{c}$ will be enhanced at LHeC
comparing to HERA. In Figs. \ref{fig:3}-\ref{fig:4} the contour
plots for the anomalous couplings in $\kappa_{u}-\kappa_{c}$ plane
are presented. For this purpose, a $\chi^{2}$ analysis is performed
\begin{eqnarray}
\chi^{2} & = & \sum_{i=1}^{N}\left({\scriptstyle {\textstyle \frac{\mbox{\ensuremath{\sigma}}_{S+B}^{i}-\mbox{\ensuremath{\sigma}}_{B}^{i}}{\Delta\sigma_{B}^{i}}}}\right)^{2}\label{eq:4}\end{eqnarray}
 where $\mbox{\ensuremath{\sigma}}_{B}^{i}$ is the cross section
for the SM background in the $i^{th}$ bin. It includes both $b$-jet
and light-jet contributions with the corresponding efficiency factors.
In the $\sigma_{S+B}$ calculations, we take into account $\kappa_{u}$
different from $\kappa_{c}$ case as well as signal-background interference.
From Figs. \ref{fig:2}-\ref{fig:4} the sensitivity is enhanced by
a factor of 1.5 when the luminosity changes from 2 fb$^{-1}$ to 10
fb$^{-1}$. Concerning the energy upgrade, increasing electron energy
from 70 GeV to 140 GeV results in 20$\%$ improvement for $\kappa_{c}$~\cite{Cakir:2009rq}.
Increasing electron energy further (energy frontier $ep$ collider)
does not give essential improvement in sensitivity to anomalous couplings
~\cite{Cakir:2003cg}.

%
\begin{figure}[hb]
\centering{\includegraphics[clip=,width=0.35\textwidth,scale=0.4]{ocakir_anomtop_fig3}\caption{Contour plot for the anomalous couplings reachable at the LHeC based
$\gamma p$ collider with the ep center of mass energy $\sqrt{s_{ep}}=1.4$
TeV and integrated luminosity $L_{int}=2$ fb$^{-1}$\label{fig:3} }}

\end{figure}

%
\begin{figure}[hb]
\centering{\includegraphics[clip=,width=0.35\textwidth,scale=0.4]{ocakir_anomtop_fig4}\caption{Contour plot for the anomalous couplings reachable at the LHeC based
$\gamma p$ collider with the ep center of mass energy $\sqrt{s_{ep}}=1.4$
TeV and integrated luminosity $L_{int}=10$ fb$^{-1}$\label{fig:4}.}}

\end{figure}


Finally the value of $\kappa/\Lambda=0.01$ TeV$^{-1}$ corresponds
to $BR(t\rightarrow\gamma u)\approx2\times10^{-6}$ which is two orders
smaller than the LHC reach with 100 fb$^{-1}.$ It is obvious that
even upgraded LHC will not be competitive with LHeC based $\gamma p$
collider in the search for anomalous $t\gamma q$ interactions. Different
extensions of the SM (SUSY, technicolor, little Higgs, extra dimensions
etc.) predict branching ratio $BR(t\rightarrow\gamma q)$=$O$(10$^{-5}$),
hence the LHeC will provide opportunity to probe these models. The
top quark could provide very important information for the Standard
Model extentions due to its large mass close to the electroweak symmetry
breaking scale. The sensitivity to anomalous coupling $\kappa/\Lambda$
could be reached down to 0.01 TeV$^{-1}$.
\clearpage



==> physics/bsm_ocakir_diquark.tex <==
\subsection{Diquarks in $\gamma p$ collisions at LHeC}

\vspace{0.2cm}
\noindent
% Orhan \c{C}ak{\i}r (Ankara Univ.) and Mehmet \c{S}ahin (TOBB) ~~~~~~~~~~~~~~~~~~ 17.08.2010

%------------------------------------
%
% Start of the text proper
%

A group theory consideration indicates that quark-quark interactions
can generate bosonic exotic color states, color-sextet and color-antitriplets.
There are theoretical motivations to consider those exotic color states,
including scalar quarks in supersymmetric (SUSY) theories with $R$-parity
violation \cite{Barbier:2004ez}, and color-sextet scalar diquarks \cite{Mohapatra:2007af}.
The diquarks were also suggested by the models beyond the Standard
Model (SM) such as composite models \cite{Terazawa:1979pj} and the superstring-inspired
$E_{6}$ models \cite{Hewett:1988xc}. In general, diquarks have scalar
and vector form and carry baryon number $|B|=2/3$, and no lepton
number. They carry electric charges $|Q|=1/3$, $2/3$ or $4/3$.
The scalar and vector diquark states of exotic quantum numbers have
been classified in Ref. \cite{Atag:1998xq,Arik:2001bc,Cakir:2005iw}.

Resonant productions of color-antitriplet scalar diquarks \cite{Atag:1998xq,Cakir:2005iw}
and vector diquarks \cite{Arik:2001bc} have been studied at the Large
Hadron Collider (LHC), linear $e^{+}e^{-}$ colliders \cite{Cakir:2005iw,Gusso:2003gz}
and $ep$ colliders \cite{Cakir:2005iw,Hewett:1988xc}. Pair production of color-sextet
scalars at the LHC has been studied in Ref. \cite{Chen:2008hh}. The next-to-leading
order QCD corrections to quark-quark annihilation to a scalar resonant
state (diquark) in a color representation of antitriplet or sextet
at the Tevatron and LHC energies are calculated in Ref. \cite{Han:2009ya}:
for the LHC, they find the enhancement (K-factor) for the color-antitriplet
diquark is about 1.31\textendash{}1.35, and for the color-sextet diquark
is about 1.22\textendash{}1.32.

The collider detector at Fermilab (CDF) has set limits on the masses
of scalar diquarks (predicted by $E_{6}$ model) decaying to dijets
with the exclusion of mass range $290<m_{DQ}<630$ GeV \cite{Aaltonen:2008dn}.
This limit is expected to be approximately valid for other scalar
diquarks. There is also indirect bounds imposed on couplings by the
electroweak precision data from LEP where these bounds allow diquark-quark
cuplings up to a value $\alpha_{DQ}$=$0.12$ \cite{Bhattacharyya:1995bw}.

We analyse the single production of scalar and vector diquarks at
the LHeC based $\gamma p$ collider. We calculate the decay widths,
differential cross sections and total cross sections of the signal,
and the corresponding background. The signal and background analysis
are performed for the diquark types of $uu$, $ud$ and $dd$. Since
the diquark exotics couple to a pair of quarks, and there is one more
associated quark in the final state, hence there appears three-jets
to deal with for the analysis. The background for three jet final
states are examined through appropriate kinematical cuts. Here, we
also discuss the possibility of measurements for the charges of diquarks
($qq$ and $qq'$) at the LHeC. The main parameters of the energy
and luminosity options for a LHeC based $\gamma p$ collider are listed
in Table \ref{diquark_tab:1}.

A model independent, baryon number conserving, general $SU(3)_{C}\times SU(2)_{W}\times U(1)_{Y}$
invariant effective lagrangian for scalar and vector diquarks has
the form \cite{Atag:1998xq,Arik:2001bc}

\begin{eqnarray}
L_{|B|=2/3}=(g_{1L}\bar{q}_{L}^{c}i\tau_{2}q_{L}+g_{1R}\bar{u}_{R}^{c}d_{R})DQ_{1}^{c}+\widetilde{g}_{1R}\bar{d}_{R}^{c}d_{R}\widetilde{DQ}_{1}^{c}\nonumber \\
+\widetilde{g'}_{1R}\bar{u}_{R}^{c}u_{R}\widetilde{DQ'}_{1}^{c}+g_{3L}\bar{q}_{R}^{c}i\tau_{2}\tau q_{L}\cdot\textbf{DQ}_{3}^{c}\hspace{0.6in}\nonumber \\
+g_{2}\bar{q}_{L}^{c}\gamma_{\mu}d_{R}DQ_{2\mu}^{c}+\widetilde{g}_{2}\bar{q}_{L}^{c}\gamma^{\mu}u_{R}\widetilde{DQ}_{2\mu}^{c}+H.c.\hspace{0.8in}\end{eqnarray}
where $q_{L}=(u_{L},d_{L})$ denotes the left-handed quark spinor
and $q^{c}=Cq^{T}(\bar{q}^{c}=-q^{T}C^{-1})$ is the charge conjugated
quark field. For the sake of simplicity, color and generation indices
are ommitted in (1). Scalar diquarks $DQ_{1}$, $\widetilde{DQ}_{1}$,
$\widetilde{DQ'}_{1}$ are $SU(2)_{W}$ singlets and $\textbf{DQ}_{3}$
is a $SU(2)_{W}$ triplet. Vector diquarks $DQ_{2}$ and $\widetilde{DQ}_{2}$
are $SU(2)_{W}$ doublets. At this stage, we assume that each SM generation
has its own diquarks and relevant couplings in order to avoid flavour
changing neutral currents. A general classification of the first generation,
color anti-triplet $(3^{*})$ diquarks is shown in Table \ref{diquark_tab:2}.

%
\begin{table}[htb]
\caption{Main parameters of energy and luminosity options of LHeC based $\gamma p$
collider. \label{diquark_tab:1}}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Collider  & $E_{e}$(TeV)  & $E_{p}$(TeV)  & $\sqrt{s_{ep}}$(TeV)  & $\sqrt{s_{\gamma p}^{max}}$  & $L_{\gamma p}^{int}\approx L_{ep}^{int}(10^{2}pb^{-1})$\tabularnewline
\hline
LHeC  & 0.07  & 7  & 1.40  & 1.28  & 10-100\tabularnewline
\hline
LHeC  & 0.14  & 7  & 1.98  & 1.80  & 10-100\tabularnewline
\hline
\end{tabular}
\end{table}
%
%
\begin{table}[htb]
\caption{Quantum numbers of the first generation, color anti-triplet diquarks
described by the effective lagrangian (1). \label{diquark_tab:2}}
\centering{}\begin{tabular}{cccccc}
 &  &  &  &  & \tabularnewline
\hline
 & SU(3)$_{C}$  & SU(2)$_{W}$  & U(1)$_{Y}$  & $Q$  & Couplings \tabularnewline
\hline
Scalar Diquarks  &  &  &  &  & \tabularnewline
$DQ_{1}$  & 3$^{\star}$  & 1  & 2/3  & 1/3  & $u_{L}d_{L}(g_{1L}),\, u_{R}d_{R}(g_{1R})$\tabularnewline
$\widetilde{DQ}_{1}$  & 3$^{\star}$  & 1  & -4/3  & 2/3  & $d_{R}d_{R}(\tilde{g}_{1R})$\tabularnewline
$\widetilde{DQ}_{1}^{\prime}$  & 3$^{\star}$  & 1  & 8/3  & 4/3  & $u_{R}u_{R}(\tilde{g}_{1R}^{\prime})$\tabularnewline
$DQ_{3}$  & 3$^{\star}$  & 3  & 2/3  & $\left(\begin{array}{c}
4/3\\
1/3\\
-2/3\end{array}\right)$  & $\left(\begin{array}{c}
u_{L}u_{L}(\sqrt{2}g_{3L})\\
\begin{array}{c}
u_{L}d_{L}(-g_{3L})\\
d_{L}d_{L}(-\sqrt{2}g_{3L})\end{array}\end{array}\right)$\tabularnewline
\hline
Vector Diquarks  &  &  &  &  & \tabularnewline
$DQ_{2\mu}$  & 3$^{\star}$  & 2  & -1/3  & $\left(\begin{array}{c}
1/3\\
-2/3\end{array}\right)$  & $\left(\begin{array}{c}
d_{R}u_{L}(g_{2})\\
d_{R}d_{L}(-g_{2})\end{array}\right)$\tabularnewline
$\widetilde{DQ}_{2\mu}$  & 3$^{\star}$  & 2  & 5/3  & $\left(\begin{array}{c}
4/3\\
1/3\end{array}\right)$  & $\left(\begin{array}{c}
u_{R}u_{L}(\tilde{g}_{2})\\
u_{R}d_{L}(-\tilde{g}_{2})\end{array}\right)$ \tabularnewline
\hline
\end{tabular}
\end{table}


We consider the color $\mathbf{3}^{*}$ scalar $DQ_{1}$ or $DQ_{3}^{0}$
diquarks coupled to $ud$ pairs, $\widetilde{DQ}_{1}$ or $DQ_{3}^{-}$
diquarks coupled to $dd$ pair and $\widetilde{DQ'}_{1}$ or $DQ_{3}^{+}$
diquarks coupled to $uu$ pair. Here, $DQ_{3}^{(+,0,-)}$ denotes
the isospin triplet component of scalar diquarks. The vector diquarks
$DQ_{2\mu}^{1}$ and $\widetilde{DQ}_{2\mu}^{2}$ couple to $ud$
pair, while $DQ_{2\mu}^{2}$ and $\widetilde{DQ}_{2\mu}^{1}$ couple
to $dd$ and $uu$ pair, respectively. 
%The decay widths for scalar
%and vector diquarks are calculated from the equation (1) and we plot
%the diquark decay width versus diquark mass in Fig. \ref{fig:ocakir_diquark_fig1}.
%We find the decay widths $\Gamma=8.75$ GeV for scalar diquarks and
%$\Gamma=5.83$ GeV for vector diquarks with $m_{DQ}=700$ GeV and
%coupling $\alpha_{DQ}=0.1$.
For a coupling $\alpha_{DQ}=0.1$, the diquark decay width ranges between $\sim 5$~GeV
and $\sim 10$~GeV for diquark masses below $1$~TeV.

%
% \begin{figure}[htb]
% \centering{\includegraphics[scale=0.7]{ocakir_diquark_fig1}
% \caption{Decay width versus mass of scalar (S) and vector (V) diquarks with
% the coupling $\alpha_{DQ}=0.1$.\label{fig:ocakir_diquark_fig1}}}
% \end{figure}


%
\begin{figure}[htb]
\centering{\includegraphics{ocakir_diquark_fig2}

\caption{Diagrams for the single production of diquarks at LHeC based $\gamma p$
collider.\label{fig:ocakir_diquark_fig2}}}

\end{figure}


The diquarks can be produced singly via the process $\gamma p\to DQqX$
(see Fig. \ref{fig:ocakir_diquark_fig2}) at the LHeC based $\gamma p$ collider,
and the cross section will be proportional to diquark charges. There
is also the possibility for charge measurement of diquarks (via $pp\to DQ\gamma X$
process) at the LHC, but it much suffers from the large 2-jet and
3-jet background. Moreover, the resonant production of diquarks dominates
at the LHC. Hence, the diquark charges can be identified at the LHeC
based $\gamma p$ collider. The signal for diquark single production
would clearly manifest itself in three jets cross sections. Given
the $uu$ or $dd$ type of diquarks there are 4 signal diagrams ($2\to3$
process) interfering with the 12 SM diagrams ($2\to3$ process) for
three-quark final states. The other three-jet final states contributes
to the background (reducible). The total cross section for the single
production of diquarks at $\gamma p$ collider is given by

\begin{equation}
\sigma_{DQ}^{S,V}=\sum_{q}\int_{M_{DQ}^{2}/s}^{0.83}d\tau\int_{\tau/0.83}^{1}\frac{dx}{x}f_{q/p}(x,Q^{2})f_{\gamma/e}(\frac{\tau}{x})\int_{\widehat{t}_{\min}}^{\widehat{t}_{\max}}d\widehat{t}\frac{d\hat{\sigma}_{DQ}^{S,V}}{d\hat{t}}\end{equation}
where $f_{q/p}(x,Q^{2})$ is the quark distribution functions from
the proton. The third integration over $\hat{t}$ is taken in the
interval $\hat{t}_{\min}$ and $\hat{t}_{\max}$, where $\hat{t}_{\min}=-\hat{s}+m_{DQ}^{2}$
and $\hat{t}_{\max}=0$. The energy spectrum of the Compton backscattered
photons from electrons is given by \begin{equation}
f_{\gamma/e}(z)=\frac{1}{D(\xi)}\left[1-z+\frac{1}{1-z}-\frac{4z}{\xi(1-z)}+\frac{4z^{2}}{\xi^{2}(1-z)^{2}}\right],\end{equation}
 with

\begin{equation}
D(\xi)=(\frac{1}{2}+\frac{8}{\xi}-\frac{1}{2(1+\xi)^{2}})+(1-\frac{4}{\xi}-\frac{8}{\xi^{2}})\ln(1+\xi),\end{equation}
where $\xi=4E_{e}\omega_{0}/m_{e}^{2},$ and $z=E_{\gamma}/E_{e}$
is the ratio of the backscattered photon energy to the initial electron
energy. The energy $E_{\gamma}$ of converted photons restricted by
the condition $z_{\max}=0.83$. The value $z_{\max}=\xi/(\xi+1)=0.83$
corresponds to $\xi=4.8$. In Fig. \ref{fig:ocakir_diquark_fig3}, we present the
photon spectrum from different sources, namely the ProtonPhoton (proton
emits photon), WWPhoton (electron emits photon) and ComptonPhoton
(conversion of electron energy to photon energy).

%
\begin{figure}[htb]
\centering{\includegraphics[scale=0.7]{ocakir_diquark_fig3}

\caption{Photon energy spectrum for different photon sources as explained in
the text. \label{fig:ocakir_diquark_fig3}}}

\end{figure}


%
\begin{table}[htb]
\caption{Cross sections for scalar $uu$ ($dd$) type diquarks in $\gamma p$
collisions available at LHeC and LHC. \label{diquark_tab:3}}
\begin{tabular}{|c|c|c|c|}
\hline
Cross sections in fb & \multicolumn{2}{c|}{LHeC($\gamma p$ coll.)} & LHC($\gamma p$ coll.)\tabularnewline
\hline
Mass (GeV) & 1.4 TeV & 1.9 TeV & 14 TeV\tabularnewline
\hline
700 & 36.56(2.53) & 189.37(18.57) & 12.23(2.04)\tabularnewline
\hline
800 & 10.04(0.58) & 93.21(8.51) & 8.61(1.32)\tabularnewline
\hline
900 & 2.31(0.12) & 42.97(3.50) & 6.65(0.85)\tabularnewline
\hline
1000 & 0.53(0.03) & 19.84(1.39) & 4.58(0.64)\tabularnewline
\hline
\end{tabular}
\end{table}


The total cross sections for scalar and vector diquarks (with mass
$m_{DQ}=700$ GeV and coupling $\alpha_{DQ}=0.1$) depending on the
electron beam energies are shown in Figure \ref{fig:ocakir_diquark_fig4}. From these
figures we find that diquarks with charge $|Q|=4/3$ have the largest
cross sections when compared to the other types. In Table \ref{diquark_tab:3},
we also compare the cross sections for single diquark photo-production
processes in the LHeC based $\gamma p$ collisions and photon-proton
collisions at the LHC.

%
\begin{figure}[htb]
\centering{\includegraphics[scale=0.6]{ocakir_diquark_fig4a} \includegraphics[scale=0.6]{ocakir_diquark_fig4b}

\caption{Total cross sections for single scalar diquark (left) and vector diquark
(right) production as a function of the electron beam energy ($E_{e}=50-250$
GeV) at $ep$ based $\gamma p$ colliders, where proton beam (from
the LHC) has an energy $E_{p}=7000$ GeV. \label{fig:ocakir_diquark_fig4}}}

\end{figure}


%
% \begin{figure}[htb]
% \centering{\includegraphics[scale=0.7]{ocakir_diquark_fig5}
% \caption{Transverse momentum distributon for scalar diquarks with $M_{DQ}=700$
% GeV at $\sqrt{s}=1.4$ TeV LHeC energy options. \label{fig:ocakir_diquark_fig5}}}
% \end{figure}


%
\begin{figure}[htb]
\centering{\includegraphics[scale=0.7]{ocakir_diquark_fig6}

\caption{Pseudo-rapidity distribution for the jets from scalar diquark production
with $M_{DQ}=700$ GeV at $\sqrt{s}=1.4$ TeV LHeC energy option.
\label{fig:ocakir_diquark_fig6}}}

\end{figure}


%
\begin{figure}[htb]
\centering{\includegraphics[scale=0.6]{ocakir_diquark_fig7}

\caption{Pseudo-rapidity distributions for SM $3jet$ background at $\sqrt{s}=1.4$
TeV LHeC energy option. \label{fig:ocakir_diquark_fig7}}}

\end{figure}


%
\begin{figure}[htb]
\centering{\includegraphics[scale=0.7]{ocakir_diquark_fig8}

\caption{Dijet invariant mass distributions for $ep\rightarrow DQjX\rightarrow jjjX$.
Resonance peaks are shown for scalar diquark masses 700, 800, 900
GeV for comparison with smooth QCD backgrounds. \label{fig:ocakir_diquark_fig8}}}

\end{figure}


We generate diquark signal and the corresponding background events
with the program CalcHEP \cite{Pukhov:1999gg,Pukhov:2004ca} using the parton distribution
functions CTEQ6M \cite{Lai:1999wy}. Here, we consider two types of background
one is interfering with the signal events and the other is reducible
background contributing to three-jet events. The background for three-jet
final state has large cross section, since the signal has different
shape than the background we have opportunity to reduce these backgrounds
by applying suitable kinematical cuts. 
% trivial...
% In Figure \ref{fig:ocakir_diquark_fig5},
%the $p_{T}$ distribution of 3 jets for signal with $M_{DQ}=700$
%GeV are shown. The jets from diquarks have large transverse momentum
%distribution around the half value of the diquark mass. Thus, 
We need
at least 20 GeV cut for the transverse momentum of all three-jets
and additional kinematics cuts to reduce background more efficiently.
In Fig. \ref{fig:ocakir_diquark_fig6}, the pseudo-rapidity distributions of jets
are presented for the signal with $M_{DQ}=700$ GeV in $\gamma p$
collisions of LHeC with $\sqrt{s}=1.4$ TeV. The signal jets from
scalar diquark are mostly located in the pseudo-rapidity $\eta\simeq2$.
In Figure \ref{fig:ocakir_diquark_fig7}, one can see the distribution of pseudo-rapidity
(mostly in the range $\eta\simeq1$) from SM three-jet background.
The invariant mass distribution of dijets from the scalar diquark
signal and the SM background are shown in Fig. \ref{fig:ocakir_diquark_fig8}. From
these figures, more appropriate cuts for signal jets are: pseudo-rapidity
$1<\eta^{j}<3$, invariant mass $m_{DQ}-\Delta m<m_{jj}<m_{DQ}+\Delta m$,
transverse momentum $p_{T}^{j}>20$ GeV at LHeC $\sqrt{s}=1.4$ TeV
energy option.

In order to obtain the observability of diquarks at LHeC based $\gamma p$
collider we have calculated the signal (S) and background (B) event
estimations for an integrated luminosity of $10$ $fb^{-1}$ for one
year of operation. For a realistic analysis of the background events
we take into account the finite energy resolution of the generic hadronic
calorimeter as $\delta E/E=0.5/\sqrt{E}+0.03$ for jets with $|y|<3$.
The corresponding two-jet invariant mass resolution is given approximately
by $\delta m_{jj}=0.5\sqrt{m_{jj}}+0.02m_{jj}$. The mass interval
is taken as $\Delta m=max(\Gamma_{DQ},\delta m_{jj})$. The significance
of signal over the background is defined as $S/\sqrt{B}$. Thus we
used relevant cuts and the detector parameters to find the observability
of diquarks at LHeC based $\gamma p$ collider. Then, we listed the
values in Table \ref{diquark_tab:5} and \ref{diquark_tab:6} where $SS$ represent
significance of diquark signal.

%
\begin{table}[htb]
\caption{Observability of scalar diquarks at $\gamma p$ collider based on
LHeC $\sqrt{s}=1.4$ TeV. \label{diquark_tab:5}}
\begin{tabular}{|c|c|c|c|}
\hline
\multicolumn{4}{|c|}{$SS$ for $L_{int}=10fb^{-1}$}\tabularnewline
\hline
$M_{DQ}$(GeV)  & $DQ(uu)$  & $DQ(ud)$  & $DQ(dd)$\tabularnewline
\hline
700  & 17.2  & 3.6  & 1.2\tabularnewline
\hline
800  & 10.1  & 1.8  & ---\tabularnewline
\hline
900  & 4.8  & ---  & ---\tabularnewline
\hline
\end{tabular}
\end{table}


%
\begin{table}[htb]
\caption{Observability of scalar diquarks at $\gamma p$ collider based on
LHeC $\sqrt{s}=1.98$ TeV. \label{diquark_tab:6}}
\begin{tabular}{|c|c|c|c|}
\hline
\multicolumn{4}{|c|}{$SS$ for $L_{int}=10fb^{-1}$}\tabularnewline
\hline
$M_{DQ}$(GeV)  & $DQ(uu)$  & $DQ(ud)$  & $DQ(dd)$\tabularnewline
\hline
700  & 36.4  & 10.8  & 3.6\tabularnewline
\hline
800  & 28.3  & 7.8  & 2.5\tabularnewline
\hline
900  & 19.9  & 5.1  & 1.6\tabularnewline
\hline
1000  & 14.9  & 3.4  & 1.0\tabularnewline
\hline
1100  & 10.4  & 2.1  & ---\tabularnewline
\hline
1200  & 6.3  & ---  & ---\tabularnewline
\hline
\end{tabular}
\end{table}


If we take at least $10$ signal events and $S/\sqrt{B}\geq3$ as
observability criteria, for the diquarks with charge $|Q|=2/3$ it
is possible to cover mass ranges up to $0.8$ TeV at the LHeC with
$L_{int}=10fb^{-1}$ and $\sqrt{s}=1.98$ TeV. The scalar diquarks
with charge $|Q|=4/3$ can be observed up to $1.2$ TeV at $\sqrt{s}=1.98$
TeV.

In conclusion, if diquarks exist the LHC could find them in resonance
channel, however their charges and coupling types can be best identified
via single production at the LHeC based $\gamma p$ collider. In the
single production mechanism, the spin of the diquarks can also be
determined by studying the angular distributions of the final state
jets \cite{Cakir09}.

\clearpage


==> physics/bsm_ocakir_fourth.tex <==
\newpage
\subsection{Single production of fourth family quarks at LHeC}
\vspace{0.2cm}
\noindent

% O.Cakir (Ankara Univ.), V. Cetinkaya (Ankara Univ.), A. Senol (Kastamonu Univ.), T. Tasci (Kastamonu Univ.) ~~~~~~~~~~~~~~~~~~ 17.08.2010

%------------------------------------
%
% Start of the text proper
%

The Large Hadron Collider (LHC) has started to scan a new range of
energy, and mass to solve the well known unanswered questions in particle
physics; especially concerned, two of them are the flavor problem
and the electroweak symmetry breaking. Furthermore, one of the questions
left open by the standard model (SM) is the replication of fermion
generations. The SM does not provide a mathematical tool to predict
the number of fermion families. One of the main aims of the present
high energy collider experiments is to determine the number of fermion
families. The possibility of existence of an extra fermion family
is under discussion \cite{Arik:1996qd,Ginzburg:1998ki,Holdom:2006mr,
Kribs:2007nz,Ozcan:2008zz,Cakir:2008su,Ciftci:2008tc,Ozcan:2009qm,
Cakir:2009ib,Erler:2010sk} at hadron colliders, recently
in the context of the LHC experiments. The LHeC would also be expected
to have sensitivity to the new quarks and leptons. The discovery of
fourth family fermions that have sequential couplings could play an
important role to understand the flavor structure of the SM. The constraints
on the fourth family depend not only on the masses of the new quarks
but also on the mass of charged lepton and neutrino as well as the
mass of the Higgs boson \cite{Erler:2010sk,Maltoni:1999ta}.

Recently, the Collider Detector at Fermilab (CDF) has already constrained
the masses of fourth family quarks: $m_{t^{\prime}}>335$ GeV at $95\%$
CL. \cite{CDF10-1}, and $m_{b^{\prime}}>338$ GeV at $95\%$ CL.
\cite{Aaltonen:2009nr} complementing the previous limits \cite{Amsler:2008zzb}.
However, there seems to be some parameter space (mass, mixing) left
for the fourth family quarks which could be investigated in the future
experiments.

Here, we investigate the discovery potential of the LHeC for the single
production of fourth family $t'$ and $b'$ quarks via the process
$e^{+}p\rightarrow t'\bar{\nu}_{e}X$ and $e^{-}p\rightarrow b'\nu_{e}X$
\cite{Cakir:2009ir}. We calculate the cross sections of signal and corresponding
backgrounds. The decay widths and branching ratios of the fourth family
$t^{\prime}$ and $b^{\prime}$ quarks are calculated in the mass
range 300-800 GeV. For the numerical calculations, we have implemented
the new interaction vertices into the CompHEP \cite{Pukhov:1999gg} package
and used the parton distribution function (PDF) CTEQ6M \cite{Pumplin:2002vw}.

The simplest extension of the SM is to add a sequential fourth family
fermions. Here, the left-handed components transform as a doublet
of $SU(2)_{L}$ and right-handed components as singlets. The fourth
family $Q^{\prime}$(=$t',b'$) quark interacts with the quarks $q_{i}$
via the exchange of SM gauge bosons $(\gamma,g,Z^{0},W^{\pm})$. The
interaction lagrangian is given by

\begin{eqnarray}
L=-g_{e}Q_{Q^{\prime}}\bar{Q^{\prime}}\gamma^{\mu}Q^{\prime}A_{\mu}-g_{s}\bar{Q^{\prime}}T^{a}\gamma^{\mu}Q^{\prime}G_{\mu}^{a}-\frac{g}{2\cos\theta_{W}}\bar{Q^{\prime}}\gamma^{\mu}\left(g_{V}-g_{A}\gamma^{5}\right)Q^{\prime}Z_{\mu}^{0}\nonumber \\
-\frac{g}{2\sqrt{2}}V_{Q'q}\bar{Q^{\prime}}\gamma^{\mu}\left(1-\gamma^{5}\right)q_{i}W_{\mu}^{-}+h.c.\end{eqnarray}
where $g_{e}$, $g$ are electroweak coupling constants, and $g_{s}$
is the strong coupling constant. The vector fields $A_{\mu}$, $G_{\mu}$,
$Z_{\mu}^{0}$ and $W_{\mu}^{\pm}$ denote photon, gluon, $Z^{0}$-boson
and $W^{\pm}$-boson, respectively. $Q_{Q^{\prime}}$ is the electric
charge of fourth family $Q^{\prime}$ quark; $T^{a}$ are the Gell-Mann
matrices. The vector and axial-vector type couplings $g_{V}$ and
$g_{A}$ of neutral weak current are defined as in the SM. Finally,
the $V_{Q'q}$ denotes the elements of extended 4 $\times$ 4 CKM
mixing matrix which are constrained by flavor physics. Here, we calculate
the decay width and branchings in the case of a new parametrization
which is well motivated in a recent study \cite{Hou:2006mx,Chanowitz:2009mz,Bobrowski:2009ng}: $|V_{t'd}|=0.0044$,
$|V_{t's}|=0.114$, $|V_{t'b}|=0.22$, $|V_{ub'}|=0.028$, $|V_{cb'}|=0.116$,
$|V_{tb'}|=0.15$, $|V_{t'b'}|=0.99$, and here we assume a mass splitting
of $|m_{t^{'}}-m_{b^{'}}|\approx50$ GeV. However, other parametrizations
are commonly used in the recent studies \cite{Ozcan:2008zz,Cakir:2009ir}.

%
\begin{table}
\caption{The total decay widths and the branching ratios of $t'$ and $b'$
quarks depending on their masses. \label{ocakir_fourth_tab1}}


\begin{tabular}{ccccc}
\hline
Mass (GeV)  & $\Gamma_{t'}$ (GeV)  & $W^{+}b$($\%$)  & $W^{+}s$($\%$)  & $W^{+}d$($\%$) \tabularnewline
\hline
300  & 0.54  & 79  & 21  & 0.03 \tabularnewline
400  & 1.29  & 79  & 21  & 0.03 \tabularnewline
500  & 2.53  & 79  & 21  & 0.03 \tabularnewline
600  & 4.38  & 79  & 21  & 0.03 \tabularnewline
700  & 6.96  & 79  & 21  & 0.03 \tabularnewline
800  & 10.39  & 79  & 21  & 0.03 \tabularnewline
\hline
\end{tabular}\begin{tabular}{ccccc}
\hline
$\Gamma_{b'}$ (GeV)  &  & $W^{-}c$($\%$)  & $W^{-}t$($\%$)  & $W^{-}u$($\%$) \tabularnewline
\hline
0.18  &  & 66  & 30  & 3.9 \tabularnewline
0.55  &  & 52  & 45  & 3.0 \tabularnewline
1.22  &  & 46  & 52  & 2.7 \tabularnewline
2.25  &  & 43  & 55  & 2.5 \tabularnewline
3.72  &  & 41  & 57  & 2.4 \tabularnewline
5.70  &  & 40  & 58  & 2.3 \tabularnewline
\hline
\end{tabular}
\end{table}


%
\begin{figure}
\centering{\includegraphics[scale=0.8]{ocakir_fourth_fig1a}$\quad$\includegraphics[scale=0.8]{ocakir_fourth_fig1b}$\quad$\includegraphics[scale=0.8]{ocakir_fourth_fig1c}$\quad$\includegraphics[scale=0.8]{ocakir_fourth_fig1d}

\caption{The diagrams (a-b) for the single production of $t^{\prime}(\bar{t^{\prime}})$
quarks, and diagrams (c-d) for $b^{\prime}(\bar{b^{\prime}})$ at
$ep$ collision.\label{ocakir_fourth_fig1}}}

\end{figure}


The relevant diagrams for the single production of $t^{\prime}(\bar{t'})$
and $b^{\prime}(\bar{b'})$ quarks are shown in Fig. \ref{ocakir_fourth_fig1}.
The total decay widths and the branching ratios of $t'$ and $b'$
quarks within the SM framework are presented in Table \ref{ocakir_fourth_tab1}.
The $b'$ quark decays to $W^{-}c$ dominantly in the mass range of
300-450 GeV, while the $W^{-}t$ channel becomes more pronounced for
the high mass region (450-800 GeV). For the given parametrization,
the $t'$ branchings remain practically unchanged with the highest
branching $79\%$ of $t'\to W^{+}b$ in the considered mass range.
In Fig. \ref{ocakir_fourth_fig2}, we show the cross sections for the single production
of the fourth generation $t^{\prime}$ and $b'$ quarks depending
on their masses at the LHeC with $\sqrt{s}=1.4$ TeV. As it can be
seen from Fig. \ref{ocakir_fourth_fig2}, the $t'$ and $\bar{t'}$ single production
cross sections are the same due to small mixing between the fourth
family and first family quarks. However, the cross sections for $b'$
and $\bar{b}'$ productions differ by about a factor 2-10 depending
on the mass in the range 300-800 GeV. The cross sections for the single
production of $t'$ and $\bar{t'}$ (or $b'$ and $\bar{b'}$) can
be added to enrich the statistics for the analysis.

%
\begin{figure}
\centering{\includegraphics{ocakir_fourth_fig2}

\caption{The total cross section for the $t'(\bar{t'})$ (solid line), the
$b'$ and $\bar{b'}$ (dashed and dotted lines) at $\sqrt{s}=1.4$
TeV. \label{ocakir_fourth_fig2}}}

\end{figure}


The kinematical distributions of the final state $c$-quark (for single
$b'$ production) or $b$-quark (for single $t'$ production) for
the signal and background can be used for the effective cut analysis
\cite{Cakir:2009ir}, here we apply $p_{T}^{q}>50$ GeV. The signal and
background show different rapidity distributions for the final state
detectable particles. We infer from the results that the missing transverse
momentum cut $p_{T}^{miss}>20$ GeV is required for the analysis.
The charm (bottom) quark hadronizes immediately after it is produced.
A charmed (bottom) jet has a secondary vertex mass around 1 GeV (4
GeV). Here, we assume one can have success for tagging the charm (bottom)
hadrons.

For the analysis we use invariant mass of the $W$-boson and heavy
quark jet system ($b$-jet or $c$-jet) in the final state. Taking
into account $W^{+}b_{jet}$ (for $t'$ signal), and $W^{-}c_{jet}$
(for $b'$ signal), we calculate the number of events in the invariant
mass interval around the $m_{Q^{\prime}}$, namely $|m_{Q^{'}}-m_{Wq}|<10-20$
GeV according to the mass and the decay width of $Q'$($\equiv t',b'$)
to obtain the visible signal over the background. In this case, a
significant reduction on the background can be obtained. In the following
equation, $\sigma_{S}$ and $\sigma_{B}$ denote signal and background
cross sections, respectively, in the selected mass bins. Assuming
the Poisson statistics, the estimations for the statistical significance
($SS$) of signal is obtained by assuming an integrated luminosity
of $L_{int}=10$ fb$^{-1}/$year

\begin{equation}
SS=\sqrt{2L_{int}\epsilon\left[\left(\sigma_{S}+\sigma_{B}\right)\ln\left(1+\sigma_{S}/\sigma_{B}\right)-\sigma_{S}\right]}.\end{equation}


The number of events for the signal ($S$) and background ($B$) processes
are calculated as $N_{S,B}=\sigma_{S,B}\epsilon_{q}L_{int}$. In Table
\ref{ocakir_fourth_tab3}, the results for the signal significances of the $t'$,$b'$
quarks are shown for $L_{int}=10$ fb$^{-1}$. Here, we assume the
$c$-tagging efficiency as $\epsilon_{c}=30\%$ and $b$-tagging efficiency
as $\epsilon_{b}=60\%$. The single production of $t'$ and $b'$
quarks can be observed at the LHeC in the mass range of 300-700 GeV
provided the current bounds on the mixings with the other families
are present. For the smaller values (half values of the current parametrization)
of the $V_{qb'}$ and $V_{t'q}$ mixings we obtain a $1\sigma$ significance
for the $t'(b')$ signal at $m_{b'}=400$ GeV.

%
\begin{table}
\caption{The statistical significance ($SS$) values calculated for the single
production $t'$(or $\bar{t}'$) at the LHeC with $\sqrt{s}=1.4$
TeV and $L_{int}=10$ fb$^{-1}$. \label{ocakir_fourth_tab2}}


\begin{tabular}{cccc}
\hline
$m_{t^{\prime}}$ (GeV)  & $\sigma_{S}$ (fb)  & $\sigma_{B}$ (fb) & $SS$ \tabularnewline
\hline
300  & $2.88\times10^{1}$ & $8.14\times10^{-1}$  & $30.5$\tabularnewline
400  & $9.92\times10^{0}$ & $2.27\times10^{-1}$  & $18.5$\tabularnewline
500  & $3.14\times10^{0}$ & $6.84\times10^{-2}$  & $10.5$\tabularnewline
600  & $1.00\times10^{0}$ & $4.35\times10^{-2}$  & $5.3$\tabularnewline
700  & $2.78\times10^{-1}$ & $1.31\times10^{-2}$  & $2.7$\tabularnewline
800 & $6.72\times10^{-2}$ & $3.65\times10^{-3}$  & $1.3$\tabularnewline
\hline
\end{tabular}
\end{table}


%
\begin{table}
\caption{The statistical significance ($SS$) values calculated for the single
production $b'$($\bar{b}'$) at the LHeC with $\sqrt{s}=1.4$ TeV
and $L_{int}=10$ fb$^{-1}$. \label{ocakir_fourth_tab3}}


\begin{tabular}{cccc}
\hline
$m_{b^{\prime}}$ (GeV)  & $\sigma_{S}$ (fb)  & $\sigma_{B}$ (fb)  & $SS$ \tabularnewline
\hline
300  & $2.08\times10^{1}$($8.63\times10^{0}$)  & $1.09\times10^{0}$($1.09\times10^{0}$)  & $16.4$($8.7$) \tabularnewline
400  & $8.17\times10^{0}$($2.36\times10^{0}$)  & $3.45\times10^{-1}$($3.52\times10^{-1}$)  & $10.7$($4.4$) \tabularnewline
500  & $3.34\times10^{0}$($6.83\times10^{-1}$)  & $1.13\times10^{-1}$($1.14\times10^{-1}$)  & $7.1$($2.3$) \tabularnewline
600  & $1.43\times10^{0}$($2.09\times10^{-1}$)  & $7.55\times10^{-2}$($7.51\times10^{-2}$)  & $4.3$($1.0$) \tabularnewline
700  & $5.71\times10^{-1}$($5.98\times10^{-2}$)  & $2.43\times10^{-2}$($2.39\times10^{-2}$)  & $2.8$($0.5$) \tabularnewline
800 & $1.94\times10^{-1}$($1.58\times10^{-2}$) & $7.08\times10^{-3}$($7.00\times10^{-3}$) & $1.7$($0.3$)\tabularnewline
\hline
\end{tabular}
\end{table}


The LHC can discover the fourth family quarks in pairs and measure
their masses with a good accuracy. Here, we have explored the potential
of the LHeC for searching for the $t'$ and $b'$ single production
in the allowed parameter space. If the fourth family quarks have large
mixing with the other families of the SM, it can be produced singly
at the LHeC with large numbers. From the single production, a unique
measurement can be performed for the family mixings with the four
families.
\clearpage



==> physics/bsm_ssultansoy_coloroctetelectron.tex <==
\newpage
\subsection{Resonant production color octet electron at the LHeC}

\vspace{0.2cm}
\noindent
M. Sahin, S. Sultansoy and S. Turkoz ~~~~~~~~~~~~~~~~~~ TOBB University of Economics and Technology, Ankara, Turkey
%------------------------------------
%
% Start of the text proper
%


A large number of {}``fundamental'' particles, as well as observable
free parameters (put by hand), in Standard Model (SM) indicate that
it is not {}``the end of story''. Physics has met similar situation
two times in the past: one was the Periodic Table of the Elements
which was clarified by Rutherford's experiment later, the other was
the hadron inflation which has resulted in quark model. This analogy
implies the preonic structure of the SM fermions (see \cite{D'Souza:1992tg}
and references therein). The preonic models predict a zoo of new particles
such as excited leptons and quarks, leptoquarks, leptogluons etc.
Excited fermions and leptoquarks are widely discussed in literature
and their searches are inseparable parts of future collider's physics
programs. Unfortunately, leptogluons did not attract necessary attention,
while they are predicted in all models with colored preons \cite{Harari:1979gi},
\cite{Fritzsch:1981zh}, \cite{Greenberg:1980ri}, \cite{Barbieri:1981cy}, \cite{Baur:1985ud},
\cite{Celikel:1998dj}. For example, in the framework of fermion-scalar
models, leptons would be a bound state of one fermionic preon and
one scalar anti-preon $l=(F\bar{S})=1\oplus8$ (both F and S are color
triplets), then each SM lepton has its own colour octet partner \cite{Celikel:1998dj}
.

Tevatron and HERA Experiments are excluded leptogluon masses of lower than $300$ GeV  \cite{Abe:1989es,Abt:1993nr,Ahmed:1994td}.
The advantage of lepton-hadron colliders is the resonant production
of leptogluons, whereas at hadron or lepton colliders they are produced
in pairs. In this context, the color octet electron are investigated at the LHeC in the article ``Resonant production color octet electron at the LHeC''\cite{Sahin:2010dd}. Below we present results of this article. Two options are considered for the Large Hadron electron Collider (LHeC): the construction of new e-ring in the LHC tunnel \cite{Dainton:2006wd} or the construction of e-linac tangentially to the LHC \cite{Schulte:2004uj}, \cite{Zimmermann:2006zs}, \cite{Zimmermann:2008zzd}, \cite{Sultansoy:2003wv}, \cite{Sultansoy:2005mn}, \cite{Akay:2009yg}. In the second options, LHeC will be thought to have two stage: LHeC1 and LHeC2, respectively. In this work and in the referance [10], electron beam energy of LHeC1 and LHeC2 are taken $E_{e^{-}}=70$ GeV and $E_{e^{-}}=140$ GeV, respectively.


\subsubsection{Interaction lagrangian, decay width and production cross section}

For the interaction of leptogluons with the corresponding lepton and
gluon we use the following Lagrangian \cite{Amsler:2008zzb}, \cite{Celikel:1998tm}:

\begin{equation}
  L=\frac{1}{2\Lambda}\underset{l}{\sum}\left\{ \bar{l}_{8}^{\alpha}g_{s}G_{\mu\nu}^{\alpha}\sigma^{\mu\nu}(\eta_{L}l_{L}+\eta_{R}l_{R})+h.c.\right\} 
\end{equation}


where $G_{\mu\nu}^{\alpha}$ is the field strength tensor for gluon,
index $\alpha=1,2,...,8$ denotes the color, $g_{s}$ is gauge coupling,
$\eta_{L}$ and $\eta_{R}$ are the chirality factors, $l_{L}$ and
$l_{R}$ denote left and right spinor components of lepton, $\sigma^{\mu\nu}$
is the anti-symmetric tensor and $\Lambda$ is the compositeness scale.
The leptonic chiral invariance implies $\eta{}_{L}$$\eta_{R}=0$.
For numerical calculations we add leptogluons into the CalcHEP program
\cite{Pukhov:1999gg}.

Decay width of the color octet electron is given by

\begin{equation}
\Gamma_{e8}=\frac{\alpha_{s}M_{e8}^{3}}{4\Lambda^{2}}
\end{equation}


In Fig. 1 the decay widths of leptogluons are presented for two scenarios,
$\Lambda=M_{e8}$ and $\Lambda=10$ TeV.


%\vspace{32cm}
%
\begin{figure}[htb]
\centering{\includegraphics[scale=0.7]{ssultansoy_coloroctetelectron_figure1}}

\caption{Leptogluon decay width via its mass for $\Lambda=M_{e8}$ and $\Lambda=10$
TeV. }

%\vspace{-20cm}

\end{figure}


The resonant $e_{8}$ production cross sections for LHeC1 and LHeC2, evaluated using CalcHEP with CTEQ6L parametrization
\cite{Stump:2003yu} for parton distribution functions, are presented in
Figs. 2 and 3, respectively.




%
\begin{figure}[htb]
\centering{\includegraphics[scale=0.7]{ssultansoy_coloroctetelectron_figure2}}

\caption{Resonant $e_{8}$ production at the LHeC1.}

\end{figure}
%\vspace{-20cm}


%\vspace{10cm}


%
\begin{figure}[htb]
\centering{\includegraphics[scale=0.7]{ssultansoy_coloroctetelectron_figure3}}

\caption{Resonant $e_{8}$ production at the LHeC2.}

\end{figure}

%\vspace{-5cm}



\subsubsection{signal and background analysis}


{\bf LHeC1 stage}

First of all, let us consider $p_{T}$ and $\eta$ distributions for
signal and background processes in order to determine appropriate
kinematical cuts. All calculations were performed at the partonic
level using CalcHEP simulation program \cite{Pukhov:1999gg} with CTEQ6l
parton distributions functions \cite{Stump:2003yu}. Hereafter the term
jet means gluon for signal and quarks ($u$, $\bar{u}$, $d$, $\bar{d}$,
$c$, $\bar{c}$, $s$, $\bar{s}$, $b$, $\bar{b}$) for background
processes. At the partonic level, the signal process is $e^{-}g\rightarrow e_{8}\rightarrow e^{-}g$
and background processes are $e^{-}q\rightarrow e^{-}q$ (through
$\gamma$ and $Z$ exchange). 

The transverse momentum distribution of final state jets for signal
at $\Lambda=10$ TeV and for background is shown in Fig. 4. It is
seen that $p_{T}>150$ GeV cut essentially reduces background, whereas
signal is almost unaffected. Figs. 5 and 6 represent pseudo-rapidity
($\eta$) distributions for electrons and jets, respectively. As seen
from figure 6, $\eta_{e^{-}}$distribution for signal and background
are not drastically different. Concerning $\eta_{j}$, most of signal
lies above $\eta=0$, whereas 99 \% of background is concentrated
in $-2<\eta_{j}<0$ region. For this reasons below we use $p_{T}>150$,
$|\eta_{e}|<4$ and $0<\eta_{j}<4$. With these cuts we present in
Fig. 7 the invariant mass distributions for signal and background.

%
\begin{figure}[htb]
\centering{\includegraphics[scale=0.7]{ssultansoy_coloroctetelectron_figure4}}

\caption{Transverse momentum distributions of final state jets for signal and
background at $\sqrt{s}=1.4$ TeV and $\Lambda=10$ TeV. }

\end{figure}


%
\begin{figure}[htb]
\centering{\includegraphics[scale=0.7]{ssultansoy_coloroctetelectron_figure5}}

\caption{Pseudo-rapidity distributions of jets for signal and background at
$\sqrt{s}=1.4$ TeV and $\Lambda=10$ TeV. }

\end{figure}


%\vspace{4cm}


%
\begin{figure}[htb]
\centering{\includegraphics[scale=0.7]{ssultansoy_coloroctetelectron_figure6}}

\caption{Pseudo-rapidity distributions of electrons for signal and background
at $\sqrt{s}=1.4$ TeV and $\Lambda=10$ TeV.}

\end{figure}


%\vspace{-5cm}


%
\begin{figure}[htb]
\centering{\includegraphics[scale=0.7]{ssultansoy_coloroctetelectron_figure7}}

\caption{$ej$ invariant mass distributions for signal and background at $\sqrt{s}=1.4$
TeV and $\Lambda=10$ TeV. }

\end{figure}


%\vspace{-5cm}


The advantage of resonant production will provide an opportunity to
probe compositeness scale will above the center of mass energy of
the collider. For statistical significance we use following formula:

\begin{equation}
SS=\frac{N_{S}}{\sqrt{N_{S}+N_{B}}}
\end{equation}


where $N_{S}$ and $N_{B}$ denote number of signal and background events, and $SS$ denote istatistical significance, respectively.

%\vspace{5cm}


The number of signal and background events for different $M_{e8}$
values are presented in Table 1 for $L_{int}=1$$fb^{-1}$. In calculating
these values, in addition to cuts given above, we have used mass windows
as $M_{e8}-2\Gamma_{e8}<M_{ej}<M_{e8}+2\Gamma_{e8}$ for $\Gamma_{e8}>10$
GeV and $M{}_{e8}$ $-20$ GeV $<M_{ej}<M_{e8}+20$ GeV for $\Gamma{}_{e8}<10$
GeV. It is seen that the resonant production of the color octet electron
will provide very clean signature for masses up to $M_{e8}\simeq1$TeV.

The reachable compositeness scale values for $L_{int}=1$ and $L_{int}=10$$fb^{-1}$are
presented in Table 2. It is seen that multi-hundred TeV scale can
be searched for $M_{e8}=500$ GeV and the increase of the luminosity
by one order gives two times higher values for $\Lambda$.

Lastly, for a given $L_{int}=1$$fb^{-1}$, the upper mass limits
for $5\sigma$ discovery at LHeC1 stage are $M_{e8}=1100$ GeV
and $M_{e8}=1275$ GeV for $\Lambda=10$ TeV and $\Lambda=M_{e8}$,
respectively.



%
\begin{table}[htb]
\begin{tabular}{|c|c|c|c|c|}
\hline 
$M_{e8},$ GeV  & \multicolumn{2}{c|}{$\wedge=M_{e8}$} & \multicolumn{2}{c||}{$\wedge=10$ TeV}\tabularnewline
\hline
\hline 
 & $S$  & $B$  & $S$  & $B$\tabularnewline
\hline 
$500$  & $1.1\times10^{7}$  & $1.1\times10^{3}$  & $3.3\times10^{4}$  & $700$\tabularnewline
\hline 
$750$  & $6.4\times10^{5}$  & $630$  & $4.2\times10^{3}$  & $280$\tabularnewline
\hline 
$1000$  & $2.2\times10^{4}$  & $\mbox{1}65$  & $250$  & $53$\tabularnewline
\hline 
$1250$  & $81$  & $6$  & $1$  & $1$\tabularnewline
\hline
\end{tabular}

\caption{Number of signal and background events for LHeC1 with $L_{int}=1$$fb^{-1}$. }

\end{table}

%
\begin{table}[htb]
\begin{tabular}{|c|c|c|}
\hline 
$M_{e8},$ GeV  & $L_{int}=1$$fb^{-1}$  & $L_{int}=10$$fb^{-1}$\tabularnewline
\hline
\hline 
$500$  & $150$ ($200$)  & $275$ ($350$)\tabularnewline
\hline 
$750$  & $65$ ($90$)  & $125$ ($160$)\tabularnewline
\hline 
$1000$  & $22$ ($30$)  & $45$ ($58$)\tabularnewline
\hline
\end{tabular}
\caption{Achievable compositeness scale $\Lambda$ in TeV units at LHeC1
for $5\sigma$ ($3\sigma$) statistical significance.}
\end{table}



{\bf LHeC2 stage}

In order to determine the corresponding cuts we present $p_{T}$,
$\eta_{j}$ and $\eta_{e}$ distributions for signal and background
processes in Figs 8, 9 and 10, respectively. The figures indicate
that significant change takes place only for $\eta_{j}$. In this
subsections we will use $p_{T}>150$, $|\eta_{e}|<4$ and $-0.5<\eta_{j}<4$.
The invariant mass distributions obtained with this cuts are given
in Fig. 11.

%
\begin{figure}[htb]
\centering{\includegraphics[scale=0.7]{ssultansoy_coloroctetelectron_figure8}}

\caption{Transverse momentum distributions of final state jets for signal and
background at $\sqrt{s}=1.98$ TeV and $\Lambda=10$ TeV. }

\end{figure}


%
\begin{figure}[htb]
\centering{\includegraphics[scale=0.7]{ssultansoy_coloroctetelectron_figure9}}

\caption{Pseudo-rapidity distributions of jets for signal and background at
$\sqrt{s}=1.98$ TeV and $\Lambda=10$ TeV. }

\end{figure}


%
\begin{figure}[htb]
\centering{\includegraphics[scale=0.7]{ssultansoy_coloroctetelectron_figure10}}

\caption{Pseudo-rapidity distributions of electrons for signal and background
at $\sqrt{s}=1.98$ TeV and $\Lambda=10$ TeV.}

\end{figure}


%
\begin{figure}[htb]
\centering{\includegraphics[scale=0.7]{ssultansoy_coloroctetelectron_figure11}}

\caption{$ej$ invariant mass distributions for signal and background at $\sqrt{s}=1.98$
TeV and $\Lambda=10$ TeV. }

\end{figure}


The numbers of signal and background events for 6 different $M_{e8}$
values are presented in Table 3 (the mass window used is the same
as the one used in previous subsection). As seen from the Table very
clean signal can be obtained up to $M_{e8}\backsimeq1500$ GeV.

The reachable $\Lambda$ scales for $5$ different mass values are
given Table 4. Comparison with Table 2 show that twofold increasing
of the electron energy results in: $1.5$ times higher values of $\Lambda$
for $M_{e8}=500$ GeV, $2$ times - for $M_{e8}=750$ GeV and $4$
times - for $M_{e8}=1000$ GeV. Moreover, multi-ten TeV scales can
be achieved for $M_{e8}=1250$ and $1500$ GeV, which are not available
at LHeC1.

Finally, for a given $L_{int}=1$$fb^{-1}$, the upper mass limits
for $5\sigma$ discovery at LHeC2 are $M_{e8}=1580$ GeV and
$M_{e8}=1775$ GeV for $\Lambda=10$ TeV and $\Lambda=M_{e8}$, respectively.

%
\begin{table}[htb]
\begin{tabular}{|c|c|c|c|c|}
\hline 
$M_{e8},$ GeV  & \multicolumn{2}{c|}{$\wedge=M_{e8}$} & \multicolumn{2}{c||}{$\wedge=10$ TeV}\tabularnewline
\hline
\hline 
 & $S$  & $B$  & $S$  & $B$\tabularnewline
\hline 
$500$  & $3.3\times10^{7}$  & $1.4\times10^{3}$  & $9.8\times10^{4}$  & $940$\tabularnewline
\hline 
$750$  & $3.9\times10^{6}$  & $1000$  & $2.6\times10^{4}$  & $445$\tabularnewline
\hline 
$1000$  & $5.0\times10^{5}$  & $630$  & $5.8\times10^{3}$  & $210$\tabularnewline
\hline 
$1250$  & $5.3\times10^{4}$  & $270$  & $980$  & $76$\tabularnewline
\hline 
$1500$  & $3.5\times10^{3}$  & $77$  & $89$  & $16$\tabularnewline
\hline 
$1750$  & $55$  & $6$  & $2$  & $1$\tabularnewline
\hline
\end{tabular}

\caption{Number of signal and background events for LHeC2 with $L_{int}=1$$fb^{-1}.$}

\end{table}


%
\begin{table}[htb]
\begin{tabular}{|c|c|c|}
\hline 
$M_{e8},$ GeV  & $L_{int}=1$$fb^{-1}$  & $L_{int}=10$$fb^{-1}$\tabularnewline
\hline
\hline 
$500$  & $245$ ($320$)  & $440$ ($570$)\tabularnewline
\hline 
$750$  & $150$ ($195$)  & $275$ ($355$)\tabularnewline
\hline 
$1000$  & $82$ ($110$)  & $155$ ($205$)\tabularnewline
\hline 
$1250$  & $41$ ($56$)  & $81$ ($107$)\tabularnewline
\hline 
$1500$  & $16$ ($23$)  & $34$ ($46$)\tabularnewline
\hline
\end{tabular}

\caption{Achievable compositeness scale $\Lambda$ in TeV units at LHeC2
for $5\sigma$ ($3\sigma$) statistical significance.}

\end{table}



\subsubsection{Conclusion}

It seems that LHeC, together with providing
necessary information on PDF's and QCD basics, could play essential
role on the BSM physics, also. Concerning color octet electrons. LHeC1
will cover $M_{e8}$ mass up to O($1200$ GeV), whereas LHeC2
will enlarge covered mass range up to O($1700$ GeV).

The discovery of $e_{8}$ at this machine, simultaneously will determine
compositeness scale. For example if $M_{e8}=500$ GeV, LHeC2
with $L_{int}=10$ $fb^{-1}$ will be sensitive to $\wedge$ up to
$570$ TeV. 

\clearpage

==> physics/tex/fwdbkwd.tex <==
\label{detector:fwdbwd}


==> summary/summary.tex <==
%
The basic concepts have been designed for an upgrade of the LHC with a
new electron beam of $60$\,GeV energy. Two configurations are considered,
a ring-ring layout (RR) with an electron
storage ring mounted on top of the LHC magnets, and a linac-ring layout (LR)
based on two $10$\,GeV
superconducting linacs arranged in a $9$\,km triple racetrack configuration
tangential to IP2. Both options are worked out in detail and both are shown
to lead to a new, TeV energy scale collider of very high luminosity.
This Large Hadron Electron Collider (LHeC)
promises to become  the second energy frontier
electron-proton collider and as such the worlds cleanest, high resolution
microscope, designed to operate synchronously with the LHC in the twenties.
A concept is also presented of a novel, large acceptance apparatus,
which using modern technology is a basis for high precision
measurements of deep inelastic scattering processes. The LHeC
has a basic electron-proton physics programme devoted to
partonic  strong and electroweak interactions and also
to the new phenomena, beyond the Standard Model of particle
physics, which are hoped to be discovered with the LHC.
The unique ion beams of the LHC provide a third major field
of exploration related to the conditions of the initial state of
the quark-gluon plasma. The report provides the necessary basis
for the technical design of the LHeC project in the coming years.


